On first-order transductions of classes of graphs

We study various aspects of the first-order transduction quasi-order on graph classes, which provides a way of measuring the relative complexity of graph classes based on whether one can encode the other using a formula of first-order (FO) logic. In contrast with the conjectured simplicity of the transduction quasi-order for monadic second-order logic, the FO-transduction quasi-order is very complex, and many standard properties from structural graph theory and model theory naturally appear in it. We prove a local normal form for transductions among other general results and constructions, which we illustrate via several examples and via the characterizations of the transductions of some simple classes. We then turn to various aspects of the quasi-order, including the (non-)existence of minimum and maximum classes for certain properties, the strictness of the pathwidth hierarchy, the fact that the quasi-order is not a lattice, and the role of weakly sparse classes in the quasi-order.

==> lines.tex <==
\newpage
\begin{comment}
	
\part{Dividing lines (again)}
\label{part:divlines}
In this summary, we consider the various dividing lines depicted in \Cref{fig:div_lines} and recall relevant results about them, showing how these results and the definitions of these dividing lines can be interpreted in the framework of the transduction quasi-order. This in turn justifies several of the parts of \Cref{fig:hierarchy}. We duplicate \Cref{fig:div_lines} here as \Cref{fig:div_lines_again} for convenience.

\begin{figure}[h]
	\centering
	\includegraphics[width=.5\textwidth]{dividing_lines}
	\caption{Main dividing lines.}
	\label{fig:div_lines_again}
\end{figure}

\part{Applications} \label{part:applications}


%We extracted from \Cref{fig:hierarchy} the main dividing lines of the transduction partial order. The resulting map of the \FO-transduction universe is depicted on \Cref{fig:div_lines}.

%For each region, it is interesting to check whether there exists a maximal class.
%
%\begin{tabular}{c|c}
%	monadic-NIP&no (BE)\\
%	bounded twin-width&yes (${\rm tww}\leq 4$)\\
%	bounded cliquewidth&trivially perfect\\
%	bounded linear cliquewidth&half-graphs\\
%	monadically stable& no (BE)\\
%	structurally bounded expansion&no (diag)\\
%	bounded stable twin-width&yes (sparse tww at most $4$)\\
%	bounded treewidth&?, equivalent to collapse of tw hierarchy\\
%	bounded pathwidth&no (no collapse)\\
%	bounded shrubdepth&no (no collapse)\\
%	bounded degree&yes (cubic)\\
%	bounded degree and tww&yes (cubic tww at most $4$)\\
%	bounded degree and tw&yes (cubic trees)\\
%	bounded degree and pw&yes (paths)\\
%	bounded degree and shrubdepth&yes (edgeless)
%\end{tabular}
\section{Local monadic dependence and local monadic stability}\label{sec:monadic-dependence-and-monadic-stability}

%\begin{itemize}
%	%\item =NIP on hereditary classes
%	\item conj FPT (monadic) model checking
%	\item no m-NIP bound (by BE)
%	\item preserved by covers
%	\item not m-NIP implies exists a transduction to all graphs with preimage of size $O(n+m)$ implies that for not m-NIP, model checking is ``monadically'' hard. 
%\end{itemize}

Dependence and stability correspond to the impossibility to define arbitrarily large \emph{powerset graphs} (that is, bipartite graphs with vertex set $[n]\cup 2^{[n]}$ where $i$ is adjacent to $I$ whenever $i\in I$) and arbitrarily large half-graphs (see \Cref{def:halfgraph}).
Further model-theoretical dividing lines may be derived by considering monadic expansions, i.e. expansions by unary predicates. We say that a class $\Cc^+$ of 
colored graphs is a \emph{monadic expansion} of a class $\Cc$ of graphs if each colored graph in $\Cc^+$ is a monadic expansion of some graph in $\Cc$. 
\begin{itemize}
	\item A class $\Cc$ of graphs is \emph{monadically dependent} if every monadic expansion of $\Cc$ is dependent;
	\item a class $\Cc$ of graphs is \emph{monadically stable} if every monadic expansion of $\Cc$ is stable.
\end{itemize}


These dividing lines are characterized by the impossibility to transduce some classes.

\begin{thm}[\cite{baldwin1985second}]
	A class $\Cc$ is \emph{monadically dependent} (or \emph{monadically NIP}) if the class of all graphs is not a transduction of $\Cc$; it is \emph{monadically stable} if the class of all half-graphs is not a transduction of $\Cc$.
\end{thm}


%\subsection{Properties characterized by transductions} \label{subsec:PropsByTrans}
%\todo[R1]{distinguish “is an FO transduction of a class…” and  ” is an FO transduction of the class…” \Add}
%The terminology arises from dependent and stable theories, roughly defined by the fact that there is no ($\FO$) formula $\phi(\bar{x};\bar{y})$ that can define arbitrary bipartite graphs (resp. arbitrarily large half-graphs) on tuples in some model. A theory is then called monadically dependent/stable if every unary expansion is dependent/stable. This is weaker than the full MSO-theory being dependent/stable, since we cannot quantify over the unary relations.


The distinction between the classical versions of these properties and their monadic variants is actually not so important in our setting, as witnessed by the following theorem.

\begin{thm}[\cite{braunfeld2022existential}]
	Let $\Cc$ be a hereditary class of graphs. Then,
\begin{itemize}
	\item $\Cc$ is monadically dependent iff $\Cc$ is dependent;
	\item $\Cc$ is monadically stable iff $\Cc$ is stable.
\end{itemize}
\end{thm}

%Moreover, when a class is known to be monadically dependent, a simple characterization of monadic stability can be given.
%\begin{thm}[\cite{nevsetril2020rankwidth}]
%	For a monadically dependent class $\Cc$ the following are equivalent:
%	\begin{enumerate}
%		\item $\Cc$ is monadically stable;
%		\item $\Cc$ is stable;
%		\item some half-graph $H$ is a semi-induced subgraph of no graph in $\Cc$.
%	\end{enumerate}
%\end{thm}



%\section{Mutual algebraicity}
%\begin{itemize}
%	\item monadic NCFP
%	\item Transduction duality with equivalence relations
%	\item = Structurally bounded degree
%	\item Tree decomposition of theory
%	\item quantifier elimination by Boolean combination of existential (starting point of extension to SBE)
%	\item related difficult questions (unbounded lcw, unbounded cw)
%	\item cubic is a maximum class. (13.2)
%	\item preserved by covers
%	\item (unlabeled) smallness is preserved
%	\item every small MA class is equivalent to a small subcubic class.
%\end{itemize}

\begin{comment}

\section{Shrubdepth}
As mentioned in the introduction, 
the quasi-order $\sqsubseteq_\MSO$ defined by monadic second-order~(\MSO) transductions is conjectured to be very simple \cite[Open Problem 9.3]{blumensath10}. Precisely, it is conjectured that this quasi-order is the chain 
\begin{equation}
	\label{eq:MSO}
\Ee\cover_\MSO
\Tt_2\cover_\MSO\ldots\cover_\MSO\Tt_n\cover_\MSO\ldots\sqsubseteq_\MSO\Pp\cover_\MSO\Tt\cover_\MSO~\Gg.\end{equation}

The notion of {\em shrubdepth} of a class of graphs
has been  introduced in \cite{Ganian2012,Ganian2017}, by relating it 
to the notion of cliquewidth similarly as
treedepth is related to treewidth.
It is based on the notion of tree model, which can  be viewed as a
very simplified (or minimalistic) analogue of a graph interpretation 
into a tree of bounded height.
%
%\begin{defi}[Tree-model]
%	\label{def:tree-model}
%	We say that a graph $G$ has a {\em tree-model of $m$ labels and depth $d$}
%	if there exists a rooted tree $T$ (of height $d$) such that 
%	\begin{enumerate}[i.]
%		\item the set of leaves of $T$ is exactly $V(G)$,
%		\item the length of each root-to-leaf path in $T$ is exactly~$d$,
%		\item each leaf of $T$ is assigned one of $m$ labels
%		(\,$T$ is {\em $m$-labelled}),%
%		\item\label{it:tree-model-edge}
%		and the existence of a $G$-edge between $u,v\in V(G)$ depends solely
%		on the labels of $u,v$ and the distance between $u,v$ in $T$.
%	\end{enumerate}
%	The class of all graphs having a tree-model of $m$ labels and depth $d$ 
%	is denoted by $\TM{d}{m}$.
%\end{defi}
%\begin{defi}[Shrubdepth]
%	\label{def:shrubdepth}
%	A class of graphs $\Cc$ has {\em shrubdepth} $d$
%	if there exists $m$ such that $\Cc\subseteq\TM dm$,
%	while for all natural $m$ it is $\Cc\not\subseteq\TM{d-1}m$.
%\end{defi}
%Note that~\Cref{def:shrubdepth} is asymptotic, as it makes sense 
%only for infinite graph classes.


The importance of shrubdepth stands in the fact that on classes with bounded shrubdepth \FO-transductions, $\MSO$-transductions, and 
$\CMSO$-transductions have the same power\footnote{In this paper, by \MSO{} and \CMSO{} we refer to monadic second order logic and counting monadic second order logic, with quantification over vertices only. These logic are sometimes refered to as $\MSO_1$ and $\CMSO_1$.}. 

\begin{thm}[follows from {\cite[Theorem 4.1]{Ganian2017}}] \label{thm:ShrubTrans}
	Let $\Cc$ be a class of graphs and let $d$ be a positive integer. The following are equivalent:
\begin{enumerate}
\item $\Cc$ has shrubdepth at most $d$;
\item $\Cc$ is an \FO-transduction of $\Tt_d$;
\item $\Cc$ is an $\MSO$-transduction of $\Tt_d$;
\item $\Cc$ is a $\CMSO$-transduction of $\Tt_d$.
\end{enumerate}
\end{thm}


Blumensath and Courcelle  \cite{blumensath10} proved that $\Tt_{d+1}$ is not a $\CMSO$-transduction of $\Tt_d$, so that
\[\Ee\sqsubset_{\CMSO}
\Tt_2\sqsubset_\CMSO\ldots\sqsubset_\CMSO\Tt_n\sqsubset_\CMSO\ldots\]

This was complemented by \cite[Theorem 4.9]{Ganian2017}, which states that  any graph class with bounded shrubdepth is transduction equivalent to some class $\Tt_d$, whether we consider \FO-transductions, \MSO-transductions, or \CMSO-transductions.
Note that this positively confirms the beginning of \eqref{eq:MSO}.
A further step toward \eqref{eq:MSO} was proved (in a strong form, as it involves \FO{} instead of \MSO) as the following duality.
\begin{thm}[\cite{shrubbery}]  \label{thm:ShrubDual}
	For every class $\Cc$ of graphs,
\begin{itemize}
	\item either $\Cc$ has bounded shrubdepth (i.e.\ there is some integer $d$ with $\Cc\equiv_\FO\Tt_d$);
	\item or the class of all paths is an \FO-transduction of $\Cc$ (i.e.\
	$\Pp\sqsubseteq_\FO\Cc$).
\end{itemize}
\end{thm}

As mentioned earlier, the notion of shrubdepth is deeply related to the notion of treedepth. This connection is witnessed by the following properties.

\begin{fact}
	Weakly sparse classes with bounded shrubdepth are exactly the classes with bounded treedepth.
\end{fact}
\begin{proof}
	This well-known fact follows, for instance, from the property that classes with bounded shrubdepth exclude some path as an induced subgraph \cite{Ganian2012}, that weakly sparse classes excluding a path as an induced subgraph also exclude some path as a subgraph \cite{GRS82}, and that classes excluding a path as a subgraph have bounded treedepth \cite{Taxi_tdepth}.
\end{proof}

The next lemma  follows\footnote{The transduction used in \cite{SBE_TOCL} uses copying. However, by moving the leaves to internal vertices, it is not difficult (using  \Cref{lem:elim_copy}, for example) to get rid of copying and to derive a transduction pairing.} from \cite{SBE_TOCL}.
\begin{lem}
	\label{lem:sparse_sd}
	For every integer $d$ and every class $\Cc$ with shrubdepth at most $d$, there exists a class $\Dd\subseteq \Tt_d$ and
	 a non-copying transduction pairing of $\Cc$ and $\Dd$. \qed
\end{lem}


%where $\cover_\MSO$ denotes the covering relation of the quasi-order, $\Ee$ is the class of edgeless graphs, $\Tt_n$ is the class of forests with depth $n$ (Hence, $\Ee=\Tt_1$), $\Pp$ is the class of all paths, $\Tt$ is the class of all trees, and $\Gg$ is the class of all graphs. 

Finally, let us mention that classes with bounded shrubdepth are the building blocks of the classes that are transductions of bounded expansion classes (or even of nowhere dense classes), as we shall see in the next section.





\section{Structural sparsity}\label{sec:structural-sparsity}

The notion behind the idea of structural sparsity is to close 
a sparse class property (that is a class of  classes of sparse graphs) under transductions \cite{SurveyND}. For instance, 
a class $\Cc$ has \emph{structurally bounded degree} if it is a transduction of a class with bounded degree, it has \emph{structurally bounded expansion} if it is a transduction of a class with bounded expansion, and  it is \emph{structurally nowhere dense} if it is a transduction of a nowhere dense class.

 These definitions may seem
somehow arbitrary at first glance. 
However, classes with structurally bounded degree are characterized by strong structural properties \cite{gajarsky2020new}, and are equivalent to the model-theoretic notion of \emph{mutual algebraicity}, which will be discussed in \Cref{sec:sbddual}. Classes with structurally bounded expansion also are characterized by strong structural properties, from which we give a sample here. We believe that this justifies  considering structural bounded expansion as a (natural) dividing line.

One of the strongest characteristic structural property of classes with structurally bounded expansion is a generalization of the characteristic property of classes with bounded expansion to admit low treedepth decompositions \cite{POMNI}.

\begin{thm}[\cite{SBE_drops,SBE_TOCL}]
	\label{thm:LSD}
	A class of graphs $\Cc$ has structurally bounded expansion if and only it admits \emph{low shrubdepth decompositions}, that is, if and only if there exists a sequence
	$\Dd_1,\dots,\Dd_i,\dots$ of classes with bounded shrubdepth and integers $C_1,\dots,C_i,\dots$ such that, for every integer $p$ and every graph $G\in\Cc$, there exists a partition $V_1\cup\dots\cup V_{C_p}$ of the vertex set of $G$ with the property that any $p$ classes induce a subgraph in $\Dd_p$:
\[
	\forall I\in\binom{[C_p]}{p}\quad G\biggl[\bigcup_{i\in I}V_i\biggr]\in\Dd_p.
\]
\end{thm}
From this characterization, it is easily derived that if $\Cc$ has structurally bounded expansion, then there exists an integer $K$ such that the vertex set of each $G\in\Cc$ can be partitioned into (at most) $K$ sets, each inducing a cograph. It follows that 
every class with structurally bounded expansion is linearly $\chi$-bounded:
\[
\forall G\in\Cc\quad \chi(G)\leq K\,\omega(G).
\]

	
An important consequence of 	
	\Cref{thm:LSD}  (for the case where $p=2$) is the following sparsification theorem.
	
\begin{thm}[Implicit in \cite{SBE_TOCL}]
	\label{thm:sparsify}
	Let $\Cc$ be a class with depth-$2$ low shrubdepth decompositions, that is, a class such that there exists a class $\Dd$ with bounded shrubdepth and an integer $C$ such that, for every graph $G\in\Cc$ there exists a partition $V_1,\dots,V_C$ of the vertex set of $G$ with the property that any (one or) two classes induce a subgraph in $\Dd$.
	
	Then, there exists a weakly sparse class $\Dd$ and (non copying) transductions $\mathsf S,\mathsf T$ such that 
	$(\mathsf S,\mathsf T)$ is a transduction pairing of $\Cc$ and $\Dd$. In particular, $\Cc\equiv_\FO^\circ\Dd$.
\end{thm}
\begin{proof}
	This follows from \Cref{fact:gluing} and the existence, for every class with bounded shrubdepth, of a non-copying pairing with a class with bounded treedepth (\Cref{lem:sparse_sd}).
\end{proof}


\begin{cor}[\cite{SBE_TOCL}]
		\label{thm:sparsifyBE}
	For every class $\Cc$ with structurally bounded expansion, there exist a class $\Dd$ with bounded expansion and (non copying) transductions $\mathsf S,\mathsf T$ such that 
	$(\mathsf S,\mathsf T)$ is a transduction pairing of $\Cc$ and $\Dd$. In particular, $\Cc\equiv_\FO^\circ\Dd$.
\end{cor}

\begin{proof}
	According to \Cref{thm:sparsify}, there exists a transduction pairing 	$(\mathsf S,\mathsf T)$  of $\Cc$ and a weakly sparse class $\Dd$, where $\mathsf S$ and $\mathsf T$ are non-copying. According to \Cref{thm:LSD}, the class~$\Dd$ admits low shrubddepth decompositions, where any $p$ classes induce a graph in a class $\Dd_p$ with bounded shrubdepth. As $\Dd$ is weakly sparse, we can require that  $\Dd_p$ is also weakly sparse. As weakly sparse classes with bounded shrubdepth have bounded treedepth \cite{Ganian2017}, we deduce that $\Dd$ admits so-called low treedepth decompositions, which characterize classes with bounded expansion \cite{POMNI}.
\end{proof}

\begin{cor}
	\label{cor:ts_BE}
	Let $\Cc$ and $\Dd$ be two classes of graphs with structurally bounded expansion. Then,
	\begin{itemize}
		\item 
	 $\Cc\sqsubseteq_\FO\Dd$ if and only if every weakly sparse transduction  of $\Cc$ is a transduction of $\Dd$;
	 \item 
	 $\Cc\sqsubseteq_\FO^\circ\Dd$ if and only if every weakly sparse non-copying transduction  of $\Cc$ is a non-copying transduction of $\Dd$. 
	 %Being a transduction of $\Cc$, the class $\Dd$ is structurally nowhere dense. 
	 \end{itemize}
\end{cor}
\begin{proof}
	If $\Cc\sqsubseteq_\FO\Dd$, then every transduction of $\Cc$ is a transduction of $\Dd$ (by composition). Conversely, assume that every weakly sparse transduction  of $\Cc$ is a transduction of $\Dd$. According to \Cref{thm:sparsifyBE}, there exists a class $\mathscr B$ with bounded expansion such that $\Cc\equiv_\FO\mathscr B$. As $\mathscr B$ is weakly sparse, we get $\mathscr B\sqsubseteq_\FO\Dd$. Hence, $\Cc\sqsubseteq_\FO\Dd$.
	
	The proof of the non-copying transduction case follows the same lines.
\end{proof}	
It would be tempting to believe that \Cref{cor:ts_BE} extends to all classes. Such a property would mean that the set of all weakly sparse classes is sup-dense in the transduction quasi-order.
 Recall that a subset $S$ of a partially ordered set $(T,\preceq)$ is \emph{sup-dense} if every $t\in T$ is the supremum of a subset of $S$.
In our setting, this condition can be rephrased as follows: a subset $\Upsilon$ of classes is sup-dense in the transduction quasi-order $\sqsubseteq$  if, for every two classes $\Cc$ and $\Dd$ we have
\[
\Cc\equiv\Dd\qquad\iff\qquad\forall \Ff\in\Upsilon\quad (\Ff\sqsubseteq\Cc)\iff(\Ff\sqsubseteq\Dd).
\]

We now prove that the set $\Sigma$ of all weakly sparse classes is not sup-dense and, thus, that \Cref{cor:ts_BE} does not extend to all classes.

\begin{fact}
	\label{fact:non-sup-dense}
	The  set $\Sigma$ is not sup-dense in the transduction quasi-order.
\end{fact}
\begin{proof}
	Let $\Cc$ be the class of all  planar graphs, and let $\Dd$ be the union of $\Cc$ and of the class~$\Hh$ of all half-graphs.
	As every transduction of $\Cc$ is monadically stable and $\Dd$ is not (as it includes $\Hh$), we have $\Cc\sqsubset\Dd$. However, according to \cite{SODA_msrw}, every weakly sparse transduction of half-graphs has bounded pathwidth. According to \Cref{lem:pl2pw}, this implies that every weakly sparse transduction of 
	$\Dd$ is a transduction of $\Cc$. As $\Cc\not\equiv\Dd$, we deduce that $\Sigma$ is not sup-dense in the transduction quasi-order.
\end{proof}



\medspace

%\begin{lem}
%	\label{lem:countBE}
%	Let $\mathscr C_1,\dots,\mathscr C_k,\dots$ be countably many classes of graphs with bounded expansion.
%	
%	Then, there exists a  class $\mathscr B$ with bounded expansion such that $\mathscr C_i\sqsubseteq_\FO^\circ \mathscr B$ holds for all $i\in\mathbb N$.
%\end{lem}
%\begin{proof}
%	Let $\mathscr B$ contain, for each $i\in\mathbb N$ the $i$-subdivision of all the graphs in $\mathscr C_i$. 
%	
%	By construction, the non-copying transduction $\mathsf T_i$ which connects vertices at distance exactly $i+1$ and keep only marked vertices is such that $\mathsf T_i(\mathscr B)\supseteq \mathscr C_i$. Thus, $\mathscr C_i\sqsubseteq_\FO^\circ \mathscr B$ holds for all $i\in\mathbb N$.
%	
%	Assume that the $k$-th subdivision $H^{(k)}$ of a graph $H$ belongs to $\mathscr B$, where $H$ has minimum degree at least $3$. Then, $H^{(k)}$ is the $i$-subdivision of some graph $H'\in\mathscr C_i$ for some $i\leq k$. It follows that 
%	$\mathscr B\,\widetilde\nabla\,k\subseteq \bigcup_{i=1}^k \mathscr C_i\,\widetilde\nabla\,k$.
%	Consequently, if all the $\mathscr C_i$'s  have bounded expansion, then $\mathscr B$ has bounded expansion.
%\end{proof}

%The previous result does not extend to uncountable families. Actually, using a diagonal argument, we get the strong negative result.

%\begin{lem}
%	The only class bounding all classes with bounded expansion is (up to equivalence) the class of all graphs.
%\end{lem}
%\begin{proof}
%	Assume $\mathscr B$ is a monadically NIP bound for all classes with bounded expansion.
%	Let $\mathsf T_d$ be the transduction where two vertices are adjacent if they are at distance exactly $d$, the domain being defined by some unary relation in the expansion.
%	To a monadically NIP hereditary class $\mathscr C$ we associate the mapping $h_{\mathscr C}\colon\mathbb N\rightarrow\mathbb N$ as follows: $h_{\mathscr C}(i)$ is the largest integer $n$ such that the exact $i$-subdivision of $K_n$ belongs to $\mathscr C$.  
%	We now consider an enumeration $\mathsf T_1,\mathsf  T_2,\dots$ of all first-order transductions (there are countably many) and let $\mathscr C_i=\mathsf T_i(\mathscr B)$. We further define $h_i=h_{\mathscr C_i}$ and the function 	$h:\colon \mathbb N\rightarrow\mathbb{N}$ defined by $h(i)=h_i(i)+1$. By subdividing edges of $K_{\omega}$ more and more (depending on the maximum label of adjacent vertices) and taking the age, we get a bounded expansion class $\mathscr D$ with $h_{\mathscr D}(i)\geq h(i)$ for every integer $i$. 
%	As $\mathscr B$ is a bound of all bounded expansion classes, there exists a transduction, say $\mathsf T_k$, such that 
%	$\mathscr D\subseteq \mathsf T_k(\mathscr B)$. However, this implies $h_{\mathscr D}(i)\leq h_k(i)$ for every integer $i$, which contradicts 
%	$h_{\mathscr D}(k)\geq h(k)=h_k(k)+1$.
%\end{proof}	
%
%\begin{lem}
%	Let $\mathscr C_1,\dots,\mathscr C_k,\dots$ be countably many classes of graphs.
%	
%	If all the classes $\mathscr C_i$ are nowhere dense,
%	then there exists a nowhere class $\mathscr B$ such that $\mathscr C_i\sqsubseteq_\FO^\circ \mathscr B$ holds for all $i\in\mathbb N$.
%	
%	If all the classes $\mathscr C_i$ have bounded expansion,
%	then there exists a  class $\mathscr B$ with bounded expansion such that $\mathscr C_i\sqsubseteq_\FO^\circ \mathscr B$ holds for all $i\in\mathbb N$.
%\end{lem}
%\begin{proof}
%	Let $\mathscr B$ contain, for each $i\in\mathbb N$ the $i$-subdivision of all the graphs in $\mathscr C_i$. 
%	
%	By construction, the non-copying transduction $\mathsf T_i$ which connects vertices at distance exactly $i+1$ and keep only marked vertices is such that $\mathsf T_i(\mathscr B)\supseteq \mathscr C_i$. Thus, $\mathscr C_i\sqsubseteq_\FO^\circ \mathscr B$ holds for all $i\in\mathbb N$.
%	
%	Assume that the $k$-th subdivision $H^{(k)}$ of a graph $H$ belongs to $\mathscr B$, where $H$ has minimum degree at least $3$. Then, $H^{(k)}$ is the $i$-subdivision of some graph $H'\in\mathscr C_i$ for some $i\leq k$. It follows that 
%	$\mathscr B\,\widetilde\nabla\,k\subseteq \bigcup_{i=1}^k \mathscr C_i\,\widetilde\nabla\,k$.
%	Consequently, if all the $\mathscr C_i$'s are nowhere dense (resp. have bounded expansion), then $\mathscr B$ is nowhere dense (resp. has bounded expansion).
%\end{proof}
%

	
%	\begin{itemize}
%	%\item connection with shrubdepth.
%%	(and a $\log n$-cover is computable in P)
%%	\item sparsifiable
%%	\item only bound is all graphs
%%	\item but BE bound for any countable set of SBE classes
%	\item quantifier elimination through Boolean combinations of existential (in a monadic expansion).
%	\item examples: map graphs, ?
%	%\item two SBE classes can be compared looking at their ws transductions. Instance of touchstone conjecture.
%\end{itemize}

%\section{Structural nowhere denseness and Monadic stability}

%\begin{itemize}
%	\item quote Podewski, Ziegler; mention superflat. 
%	\item SND and LSD, computability in P.
%	\item \FO-model checking
%	\item nice toy example for Conj 17.2: is every class with locally bounded shrubdepth SND? (later, after locality)
%	\item =stable on hereditary classes
%	\item m-Stable is  preserved by covers
%\end{itemize}

A class is \emph{structurally nowhere dense} if it is a transduction of a nowhere dense class. Structurally nowhere dense classes inherit the efficient model checking properties of nowhere dense classes~\cite{grohe2014deciding} as shown in~\cite{DreierMS23}.

%\Cref{lem:countBE} is easily translated to the nowhere dense case.
%
%\begin{lem}
%	\label{lem:countND}
%	Let $\mathscr C_1,\dots,\mathscr C_k,\dots$ be countably many nowhere dense classes of graphs.
%	
%	Then, there exists a nowhere dense class $\mathscr B$ such that $\mathscr C_i\sqsubseteq_\FO^\circ \mathscr B$ holds for all $i\in\mathbb N$.
%\end{lem}
%\begin{proof}
%	Let $\mathscr B$ contain, for each $i\in\mathbb N$ the $i$-subdivision of all the graphs in $\mathscr C_i$. 
%	
%	By construction, the non-copying transduction $\mathsf T_i$ which connects vertices at distance exactly $i+1$ and keep only marked vertices is such that $\mathsf T_i(\mathscr B)\supseteq \mathscr C_i$. Thus, $\mathscr C_i\sqsubseteq_\FO^\circ \mathscr B$ holds for all $i\in\mathbb N$.
%	
%	Assume that the $k$-th subdivision $H^{(k)}$ of a graph $H$ belongs to $\mathscr B$, where $H$ has minimum degree at least $3$. Then, $H^{(k)}$ is the $i$-subdivision of some graph $H'\in\mathscr C_i$ for some $i\leq k$. It follows that 
%	$\mathscr B\,\widetilde\nabla\,k\subseteq \bigcup_{i=1}^k \mathscr C_i\,\widetilde\nabla\,k$.
%	Consequently, if all the $\mathscr C_i$'s  are nowhere dense, then $\mathscr B$ is nowhere dense.
%\end{proof}


Nowhere dense classes are have been characterized by the existence of low treedepth decompositions with $n^{o(1)}$ colors \cite{nevsetvril2011nowhere} (instead of a bounded number of colors for the characterization of classes with bounded expansion), where $n$ is the number of vertices of the considered graph in the class. This suggests that an analog of \Cref{thm:LSD} should hold for structurally nowhere dense classes.
Up to now, only one implication is known.
\begin{thm}[\cite{dreier2022treelike}]
	Let $\Cc$ be a structurally nowhere dense class of graphs.
	Then, $\Cc$ admits \emph{quasi-bounded low shrubdepth decompositions}, that is, there exists a sequence
	$\Dd_1,\dots,\Dd_i,\dots$ of classes with bounded shrubdepth and functions $f_1,\dots,f_i,\dots$ with \mbox{$f_i(x)=x^{o(1)}$} such that, for every integer $p$ and every graph $G\in\Cc$, there exists a partition $V_1\cup\dots\cup V_{f_p(|G|)}$ of the vertex set of $G$ with the property that any $p$ classes induce a subgraph in $\Dd_p$:
	\[
	\forall I\in\binom{[f_p(|G|)]}{p}\quad G\biggl[\bigcup_{i\in I}V_i\biggr]\in\Dd_p.
	\]
\end{thm}

\end{comment}

%It has been further conjectured that nowhere dense classes capture the full complexity of monadically stable classes.
\begin{comment}
\def\xx{\cite[Conjecture 6.1]{nevsetril2020rankwidth}}
\begin{conj}[\xx]
	A class of graphs is monadically stable if and only if it is structurally nowhere dense.
\end{conj}


\section{Cliquewith and linear cliquewidth}
The notion of \emph{cliquewidth} has been introduced as a dense analog of treewidth, in a hope to capture the classes where monadic second order logic is tractable \cite{courcelle1993handle}. It is defined as the minimum number of labels needed to construct a graph by means of four specific operations (label creation, disjoint union, by-label edge creation, label renaming).

\begin{exa}
	The class of grids has unbounded cliquewidth (as it is weakly sparse and has unbounded treewidth).
\end{exa}

In our setting, it will be useful to use the following characterization in terms of \FO-transductions:
\begin{thm}[\cite{colcombet2007combinatorial}]
A class $\Cc$ has bounded cliquewidth if it is an \FO-transduction of the class $\TP$ of trivially perfect graphs.
\end{thm}

The connection with treewidth is witnessed by the following property.
\begin{thm}[\cite{Gurski2000}]
  a class has bounded treewidth if  and only if it has bounded cliquewidth and it is weakly sparse.
\end{thm}

A variant of cliquewidth has been proposed, called \emph{linear cliquewidth}, where the disjoint union operation is replaced by the operation of adding an isolated labeled vertex. 
Classes with bounded linear cliquewidth also have a nice characterization in terms of \FO-transductions.
\begin{thm}[\cite{colcombet2007combinatorial}]
	A class $\Cc$ has bounded linear cliquewidth if it is an \FO-transduction of the class $\Hh$ of half-graphs.
\end{thm}

Linear cliquewidth can be seen as a dense analog of pathwidth.
\begin{thm}[\cite{Gurski2000}]
	A class has bounded pathwidth if  and only if it has bounded linear cliquewidth and it is weakly sparse.
\end{thm}


\begin{exa}
	Any hereditary class that contains some  subdivision of each cubic tree has unbounded linear cliquewidth
\end{exa}
\begin{proof}
As subdivisions of trees are weakly sparse, the unboundedness of linear  cliquewidth follows from the unboundedness of pathwidth.
\end{proof}


For classes with bounded (linear) cliquewidth, the notions of monadic stability and of structural sparsity collapse.

\begin{thm}
	\label{thm:stcw}
	A monadically stable class of graphs has
	\begin{enumerate}
		\item bounded linear cliquewidth iff it is a transduction of a class with bounded pathwidth \cite{SODA_msrw,msrw};
		\item bounded cliquewidth  iff it is a transduction of a class with bounded treewidth \cite{nevsetril2020rankwidth}.
	\end{enumerate}
\end{thm}

We shall see that this last theorem extends to classes with bounded twin-width.

\section{Twin-width}
The original definition of twin-width \cite{twin-width1} relies on so-called \emph{contraction sequences} and is purely graph theoretic. Among the numerous characterization of classes with bounded twin-width, 
one fits particularly to our setting

\begin{thm}[\cite{Tww_ordered}]
	A class $\Cc$ of graphs has bounded twin-width if and only if it is possible to linearly order the vertex set of each of the graphs in $\Cc$,  in such a way that the obtained class  of \emph{ordered graphs} is monadically dependent.
\end{thm}

Another characterization can also be given in terms of permutation classes.

\begin{thm}[\cite{TWWP-arxiv}] 
	A class of graphs has bounded twin-width if and only if it is a transduction of a class of permutations avoiding some pattern.
\end{thm}

%\textcolor{red}{
%\begin{itemize}
%	\item pol $\chi$-bounded 
%%\item closure by lexicographic product ?
%%\item \FO-model checking modulo contraction sequence or order expansion
%%\item cubic is not the unique min class with unbounded tww. (solving conj. 66 in Tww VIII)
%%\item maximum class (collapse of tww)
%\item duality between ${\rm tww}\leq 4$  and some small class $\Dd$ of subcubic graphs.
%\end{itemize}}
\begin{exa}
The class of planar graphs and the class of unit interval graphs have bounded twin-width, while the class of cubic graph does not \cite{twin-width1}.	
\end{exa}


An analog of \Cref{thm:stcw} has been proved for twin-width.
\begin{thm}[\cite{gajarsky2022stable}]
	A monadically stable class has bounded twin-width if and only if it is a transduction of a class with bounded expansion and bounded twin-width.
\end{thm}

To complement monadic dependence and monadic stability, we propose to introduce the notion of monadically straight classes:
a class $\Cc$ is \emph{monadically straight} if the class of all trivially perfect graphs is not a transduction of $\Cc$. We believe that monadic straightness could well be an important dividing line
in the transduction quasi-order (and maybe from a general model theoretical point of view).


%Some properties can be defined both ways. For instance:
%\begin{itemize}
%	\item A class $\Cc$ has \emph{bounded twin-width} if and only if it is a transduction of a proper permutation class~\cite{TWWP-arxiv} or, equivalently, each graph $G$ in $\Cc$ can be expanded into an ordered graph $G^<$ (by adding a new binary relation defining a linear order on the vertex set) in such a way that the class $\{G^<\colon G\in \Cc\}$ is monadically dependent~\cite{Tww_ordered}.
%\end{itemize}


%These properties are highlighted in \Cref{fig:hierarchy}.




%
%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%A \emph{non-copying transduction} $\mathsf{T}$ (of graphs in graphs)
%is a pair $(\Sigma_{\mathsf T},\mathsf I_{\mathsf T})$, where
%$\Sigma_{\mathsf T}$ is a finite set of unary relation symbols and
%$\mathsf I_{\mathsf T}$ is a simple interpretation of graphs in
%$\Sigma_{\mathsf T}$-colored graphs.
%For a graph $G$, we denote by $\Gamma_{\Sigma_{\mathsf T}}$ the set of all $\Sigma_{\mathsf T}$-expansions of $G$.
%%\item 
%A graph $H$ is a \emph{$\mathsf{T}$-transduction} of a graph $G$ if
%there exists a $\Sigma_{\mathsf T}$-expansion $G^+$ of~$G$ with
%$\mathsf I_{\mathsf{T}}(G^+)=H$. We denote by $\mathsf T(G)=\mathsf I_{\mathsf T}\circ \Gamma_{\Sigma_{\mathsf T}}(G)=\{\mathsf I_{\mathsf T}(G^+): G^+\in \Gamma_{\Sigma_{\mathsf T}}(G)\}$ the set of all $\mathsf{T}$-transductions of $G$.
%For a class $\Dd$ we further define $\mathsf T(\Dd)=\bigcup_{G\in\Dd}\mathsf T(G)$.
%\item 
%A class $\Cc$ of graphs is a {\em $\mathsf T$-transduction} of a class
%$\Dd$ of graphs if for every graph $H\in\Cc$ there exists a graph
%$G \in\Dd$ such that $H$ is a $\mathsf T$-transduction in $G$. 
%We also say that $\mathsf{T}$ encodes $\Cc$ in $\Dd$. 
%A class $\Cc$ of graphs is a {\em transduction} in a class $\Dd$ of
%graphs if it is a {\em $\mathsf T$-transduction} in~$\Dd$ for some
%transduction $\mathsf T$.
%%\end{trivlist}
%%\end{definition}
%Note that non-copying transductions compose, and that the relation
%``$\Cc$ is a non-copying transduction in $\Dd$'' defines a quasi-order
%on classes of graphs that we denote by
%$\Cc\sqsubseteq^{\circ}_\FO\Dd$.
%% the property that~$\Cc$ is a non-copying transduction of $\Dd$. 
%%
%%\begin{definition}
% A
%\emph{transduction} is the composition of a copy operation and a
%non-copying transduction, that is the composition of a copy operation, a coloring operation, and a simple interpretation.
%%\end{definition}
%%
%For a graph $G$ and a transduction $\mathsf T$ we write
%$\mathsf T(G)$ for the set all graphs that can be obtained as a
%$\mathsf T$-transduction of $G$, and
%for a class $\Dd$  we define
%$\mathsf T(\Dd)=\bigcup_{G\in\Dd}\mathsf T(G)$.  We say that a
%transduction $\mathsf T'$ \emph{subsumes} a transduction $\mathsf T$
%if for every graph $G$ we have
%$\mathsf T'(G)\supseteq\mathsf T(G)$. We denote by
%$\mathsf T'\geq\mathsf T$ the property that $\mathsf T'$ subsumes
%$\mathsf T$.
%%
%The following fact is easy to establish (see for instance
%\cite{SBE_drops}).
%\begin{fact}
%\label{fact:copyfirst}
%Every transduction $\mathsf T$ is subsumed by the composition of a
%single copy operation followed by a single non-copying transduction.
%\end{fact} 
%
%Hence, the relation ``$\Cc$ is a transduction in $\Dd$'' defines a
%quasi-order on classes of graphs that we denote by
%$\Cc\sqsubseteq_\FO\Dd$.
%% the property that $\Cc$ is a transduction of $\Dd$. 
%Intuitively, if $\Cc\sqsubseteq_\FO \Dd$, then $\Cc$ is at most as complex as $\Dd$.
%%We further denote by $[\Cc]_\FO$ the equivalence class of $\Cc$ in the $\sqsubseteq_\FO$ quasi-order.
%


%\end{definition}
%
%
% This observation justifies that we shall mainly study non-copying
% transductions in this paper.
%
%We recall the following definition we gave in the introduction.
%\begin{definition}
%  Let $\mathsf{T},\mathsf{T'}$ be non-copying transductions
%  respectively associated to interpretations $\mathsf I$
%  and~$\mathsf I'$. We say that $\mathsf T'$ \emph{subsumes}
%  $\mathsf T$ if, for every graph $G$ and every coloring $G^+$ of $G$
%  there is a coloring $G^*$ of $G$ such that
%  $\mathsf I'(G^*)=\mathsf I(G^+)$.
%\end{definition}
%
%
%\begin{definition}
%\label{def:trans}
%A {\em transduction} $\mathsf T$ from $\Sigma$-structures to
% $\Sigma'$-structures is defined by a simple interpretation
% $\mathsf I_{\mathsf T}$ of $\Sigma'$ in $\Sigma^+$-structures, where
% $\Sigma^+$ is a signature obtained from $\Sigma$ by adding some
% unary relations.
%
% We say that a $\Sigma'$-structure $\strB$ is a {\em
	% $\mathsf T$-transduction} of a $\Sigma$-structure $\strA$ if there
% exists a monadic lift $\strA^+$ of $\strA$ (where $\strA^+$ is a
% $\Sigma^+$-structure) with $\mathsf I_{\mathsf T}(\strA^+)=\strB$.
%
% A class $\Dd$ of $\Sigma'$-structures is a {\em
	% $\mathsf T$-transduction} of a class $\Cc$ of $\Sigma$-structures
% if, for every structure $\strB\in\Dd$ there exists a structure
% $\strA\in\Cc$ such that $\strB$ is a $\mathsf T$-transduction of
% $\strA$. We also say that $\mathsf T$ is a transduction from $\Cc$
% onto $\Dd$.
%
% A class $\Dd$ of $\Sigma'$-structures is a {\em transduction} of a
% class $\Cc$ if it is a {\em $\mathsf T$-transduction} of $\Cc$ for
% some transduction $\mathsf T$.
%%\end{definition}
%
%
%
% It will be convenient to define, for each non-negative integer $r$,
% a formula $\delta_r(x,y)$ such that $\delta_r(x,y)$ holds in a graph
% exactly when the distance of $x$ and $y$ is the graph is at most
% $r$. We define these formulas by induction:
%\begin{align*}
%	\delta_0(x,y)&:=(x=y),\\
%	\delta_1(x,y)&:=(x=y)\vee E(x,y),\\
%	\delta_i(x,y)&=(\exists z)\ (\delta_{\lfloor
	%	i/2\rfloor}(x,z)\wedge\delta_{\lceil i/2\rceil}(z,y))\quad\text{if $i>1$.}
%\end{align*} 
%Note that, for $i\geq 1$, the quantifier rank of $\delta_i$ is
% $\lceil\log_2 i\rceil$.
%
%\begin{definition}
\end{comment}

\input{local}





==> order.tex <==
\begin{comment}
\part{Structural properties of the transduction quasi-orders}
\label{sec:structural-prop}

We now study the structural properties of the transduction quasi-orders.
Many properties will be similar when considering $\sqsubseteq_\FO$ and $\sqsubseteq_\FO^\circ$. To avoid unnecessary repetitions of the statements and arguments, we shall use
the notations $\sqsubseteq,\sqsubset,\equiv$ to denote either $\sqsubseteq_\FO^\circ,\sqsubset_\FO^\circ,\equiv_\FO^\circ$ or $\sqsubseteq_\FO,\sqsubset_\FO,\equiv_\FO$.
In the following, we say that two classes $\Cc_1$ and $\Cc_2$ are \emph{equivalent} (resp.\ \emph{non-copying equivalent}, resp.\ \emph{copying equivalent}) if $\Cc_1\equiv\Cc_2$ (resp.\
$\Cc_1\equiv_\FO^\circ\Cc_2$, resp.\ $\Cc_1\equiv_\FO \Cc_2$).
Note that non-copying equivalent implies equivalent, and equivalent implies copying-equivalent.

%\todo[R2]{The paragraph starting with "For two classes" is incomprehensible. In particular, am I supposed to see all the (transduction?) equivalences? Please remind the reader of the notions "addable" and "additive".}
Recall that, for two classes $\Cc_1$ and $\Cc_2$, we defined $\Cc_1+\Cc_2=\{G_1\union G_2: G_1\in\Cc_1, G_2\in\Cc_2\}$.
 Note that $\Cc_1+\Cc_2$ is 
 a perturbation\footnote{$G_1+G_2$ can be transformed into $G_1\union G_2$ (and vice-versa) by marking $A$ the vertices in $G_1$, marking $B$ the vertices in $G_2$, and flipping the edges between $A$ and $B$.} of  $\{G_1+G_2: G_1\in\Cc_1, G_2\in\Cc_2\}$ (hence
is non-copying equivalent to it).
Also note that, by our general assumptions, both $\Cc_1$ and $\Cc_2$ contain the empty graph. Thus, $\Cc_1\cup\Cc_2\subseteq \Cc_1+\Cc_2$. 

Recall that a class $\Cc$ is \emph{addable} if $\Cc+\Cc=\Cc$, and \emph{$\equiv$-additive} (or simply \emph{additive}) if $\Cc+\Cc\equiv\Cc$.
Moreover, as  $\Cc\equiv\Dd$ implies $\Cc+\Cc\equiv\Dd+\Dd$ (as follows from \Cref{fact:triv_gluing}), every class equivalent to an addable class is additive. 

\begin{exa}
	The class of all planar graphs is addable.
	Indeed, the disjoint union of two planar graphs is planar.
	
	The class of all paths is not addable, but it is equivalent to its closure by disjoint union, hence is additive.
	Indeed,  the class of all paths is $\equiv_\FO^\circ$-equivalent to its hereditary closure (as witnessed by the hereditary transduction $\mathsf H$), which is the class of all linear forests, that is the closure of the class of all paths by disjoint union.
	
	The class of all stars  is not addable,  not equivalent to its closure by disjoint union, 	but it is equivalent to an addable class, hence is additive.
	Indeed, the class of all stars is (non-copying) equivalent to the class $\Ee$ of all edgeless graphs, which is addable. However, the class of all stars (which is equivalent to the class $\Ee$ of all edgeless graphs) is not equivalent to its closure by disjoint union (which is the class $\Tt_2$ of all star forests).

%
%The last example is less trivial. It is a bounded expansion class $\Cc$ that is not equivalent to an addable class, though it is additive.
%The class $\Cc$ contains graphs $K_0'\subseteq_i K_1'\subseteq_i\dots$, where $K_0'$ is the graph with a single vertex $v_0$, and, for $i\geq 1$, $K_i'$ is obtained from $K_{i-1}'$ by adding a vertex $v_i$ linked to all the vertices $v_j$ (with $0\leq j<i$) by paths of length $i$. 
%As $\Cc$ is a chain for the induced subgraph relation, in order to prove that $\Cc$ is additive, it is sufficient to prove that there is a transduction $\mathsf T$ such that, for every $n\in\mathbb N$ we have $K_n'\uplus K_n'\in \mathsf T(K_{2n+1}')$. For $0\leq i\leq n$, we mark one vertex over two on the path from $v_{2i}$ to $v_{2j}$ (with mark $A$)  and on the path from $v_{2i+1}$ to $v_{2j+1}$ (with mark $B$).
%We further mark $A$ all the $v_{2i}$'s and $B$ all the $v_{2i+1}$'s.
%The transduction keeps only the marked vertices, two of them being adjacent if they are marked the same way and if, in $K_{2n+1}'$, they are either adjacent or have a common neighbor that is not marked.
%It is easily checked that, this way, the transduction produces $K_n'\uplus K_n'$ from $K_{2n+1}'$.
%We now prove that $\Cc$ is not equivalent to an addable class. Assume for contradiction that $\Cc$ is equivalent to an additive class $\Dd$. Similarly, we get that the class $\Cc$ \dnnc. 
%Let $\mathsf T_1$ be a non-copying transduction such that $\Dd\subseteq \mathsf T_1(\Cc)$. According to \Cref{crl:slunion} we can assume that $\mathsf T_1$ is immersive. Hence, there exists positive integer $r$  such that  if $H\in\mathsf T_1(G)$ and $x,y\in V(H)$, we have
%	${\rm dist}_H(x,y)\geq {\rm dist}_G(x,y)/r$.
%Consequently, the degree ${\rm d}_H(x)$ of $x$ in $G$ is at most $|B_r^G(x)|$. Thus, if ${\rm d}_H(x)>2r+1$, then $x\in B_r^G(v_i)$, for some $i$. Let $S$ be the subset of the vertices of $H$ with degree greater than $2r+1$. It follows that, for every integer $R$, there is
%a subset $S_R$ of $S$ of size $f(R)$ such that the subgraph of $H^R$ induced by $S\setminus S_R$ contains no connected component of size greater than  
\end{exa}
Note that there exist additive classes that are not equivalent to addable classes. We did not include such an example, as the proof is a bit too long.


%For instance,  the class of all stars (non-copying equivalent to the class of edgeless graphs) and the class of all paths (non-copying equivalent to the class of all linear forests) are $\equiv_\FO^\circ$-additive, thus additive (for any choice of $\equiv$).  
Note that additivity is a property preserved by  equivalence ($\Cc$~additive and $\Cc'\equiv\Cc$ implies $\Cc'$ additive) and that 
if $\Cc_1$ and $\Cc_2$ are additive then $\Cc_1+\Cc_2$ is also additive.
  It is worth mentioning that $\equiv_\FO$-additive classes may be equivalently defined as classes with the \emph{joint encoding property}, that is as classes $\Cc$ such that there exists a transduction $\mathsf T$  with the property
\[
\forall G_1,G_2\in\Cc\quad \exists U\in \Cc\quad\{G_1,G_2\}\subseteq\mathsf T(U).
\]


In this section we will consider the quasi-orders $\sqsubseteq_\FO^\circ$ and $\sqsubseteq_\FO$, as well as their restrictions to the (corresponding) additive classes.
%if it is closed under disjoint union, i.e. $G_1,\G_2\in\Cc$ implies $G_1\union G_2\in\Cc$.
Let $\mathfrak C$ be the collection of all (infinite) graph classes, and let $\mathfrak A$ (resp.\ $\mathfrak A^\circ$, resp.\ $\mathfrak A^\bullet$) be the collection of all (infinite) additive (resp.\ $\equiv_\FO^\circ$-additive, resp.\ $\equiv_\FO$-additive) graph classes. (Note that $\mathfrak A$ depends on the choice of $\equiv$, hence does not represent a set of classes of graphs \emph{per se}.)
%
%For a given  $\sqsubseteq$ we consider  two quasi-orders: $(\mathfrak C,\sqsubseteq)$, on the collection of all classes of finite graphs, and $(\mathfrak A,\sqsubseteq)$ on the collection of all additive classes of finite graphs.
While speaking about these quasi-orders,  we will implicitly consider their quotients by the equivalence relation $\equiv$, which are partial orders. For instance, when we say that  $(\mathfrak C,\sqsubseteq)$ is a join-semilattice, we mean that  $(\mathfrak C\,/\equiv,\sqsubseteq)$ is a join-semilattice. Recall that a \emph{join-semilattice} is a partial order in which every two elements $a$ and $b$ have a \emph{join} (i.e. a \emph{least upper bound}) $a\vee b$. 
The cover symbol $\cover$  will always be used with reference to $(\mathfrak C,\sqsubseteq)$, $\Cc\cover\Dd$ expressing that there exists no class $\Ff$ with $\Cc\sqsubset\Ff\sqsubset\Dd$. When we shall consider covers in $(\mathfrak A,\sqsubseteq)$ we will say explicitly that $(\Cc,\Dd)$ is a cover in $(\mathfrak A,\sqsubseteq)$, expressing that there exists no additive class $\Ff$ with $\Cc\sqsubset\Ff\sqsubset\Dd$.


In~\Cref{fig:lattice}	we gave a small example of $13$ classes on which the transduction order$(\mathfrak{C},\sqsubseteq_\FO)$ forms a distributive lattice (see~\Cref{fig:lattice}) and left open whether the whole poset~$(\mathfrak{C},\sqsubseteq_\FO)$  is a distributive lattice. 
We now give a negative answer to this question, by making use of the property that the class of planar graphs transduces every class of bounded pathwidth (\Cref{sec:encoding-classes-with-bounded-pathwidth-in-the-class-of-planar-graphs}).
%This also shows that the join of infinitely many classes is not generally defined, as we could then define the meet of two classes as the join of all classes below both.

\begin{thm}
	\label{thm:nolattice}
	Neither $(\mathfrak{C},\sqsubseteq_\FO)$,  $(\mathfrak{C},\sqsubseteq_\FO^\circ)$, 
	$(\mathfrak{A}^\bullet,\sqsubseteq_\FO)$, 
	nor  $(\mathfrak{A}^\circ,\sqsubseteq_\FO^\circ)$ is a lattice.
	In particular, the (additive) class of half-graphs $\Hh$ and the (additive) class $\Pl$ of planar graphs have no greatest lower bound in these quasi-orders.
\end{thm}
\begin{proof}
		Consider one of the quasi-orders $(\mathfrak{C},\sqsubseteq_\FO)$,  $(\mathfrak{C},\sqsubseteq_\FO^\circ)$, 
		$(\mathfrak{A}^\bullet,\sqsubseteq_\FO)$, 
		or  $(\mathfrak{A}^\circ,\sqsubseteq_\FO^\circ)$, which we will denote by $(\mathfrak{X},\sqsubseteq)$.
	Assume $\Cc$ is the greatest lower bound of $\Hh$ and $\Pl$ in~$(\mathfrak{X},\sqsubseteq)$.
	According to~\Cref{thm:adler}, the class $\Pl$, being nowhere dense, is monadically stable. Thus, as $\Cc$ is (by assumption) a transduction of $\Pl$, it is also monadically stable. Hence, according to \cite{SODA_msrw}, there exists an integer $k$ such that $\Cc\sqsubseteq_\FO^\circ\PW_k$ (hence $\Cc\sqsubseteq\PW_k$). According to \Cref{thm:PW}, 
	$\PW_{k+1}\not\sqsubseteq_\FO\PW_k$ (hence $\PW_{k+1}\not\sqsubseteq\PW_k$). Thus,
	 $\Cc\sqsubset\PW_{k+1}$. However, $\PW_{k+1}$ is addable (hence additive), $\PW_{k+1}\sqsubseteq_\FO^\circ\Hh$ and, according to \Cref{lem:pl2pw},
	$\PW_{k+1}\sqsubseteq^\circ\Pl$.
	In particular, $\PW_{k+1}\in\mathfrak{X}$, $\PW_{k+1}\sqsubseteq\Hh$, and $\PW_{k+1}\sqsubseteq\Pl$, 
	what contradicts the assumption that $\Cc$ is the greatest lower bound of $\Hh$ and $\Pl$ in $(\mathfrak{X},\sqsubseteq)$.
\end{proof}

However, we shall prove in this Section that all the four transduction quasi-orders \mbox{$(\mathfrak{C},\sqsubseteq_\FO)$},  $(\mathfrak{C},\sqsubseteq_\FO^\circ)$, 
$(\mathfrak{A},\sqsubseteq_\FO)$, 
and $(\mathfrak{A},\sqsubseteq_\FO^\circ)$ are distributive join-semilattices.

In our setting, being a join-semilattice means that for every two classes $\Cc_1$ and $\Cc_2$ there exists a class $\Cc_1\wedge \Cc_2$ such that:
\begin{itemize}
	\item both $\Cc_1$ and $\Cc_2$ can be encoded in (i.e.\ are transductions of) $\Cc_1\vee\Cc_2$;
	\item if both $\Cc_1$ and $\Cc_2$ can be encoded in a class, then so does also $\Cc_1\vee\Cc_2$.
\end{itemize}
This situation can be depicted as follows, where dotted lines represent $\sqsubseteq$ (the lower element being smaller than or equal to the upper element).
\[
\xymatrix@R=20pt@C=20pt{
	&\Dd\ar@{..}[dl]\ar@{..}[dr]&&&&\Dd\ar@{..}[d]&\\
	\Cc_1&&\Cc_2&\Longrightarrow&&\Cc_1\vee\Cc_2\ar@{..}[dl]\ar@{..}[dr]&\\
	&&&&\Cc_1&&\Cc_2\\
}
\]

A join-semilattice is \emph{distributive}
if, for all elements $a,b,x$ with $x\leq a\vee b$ there exists $a'\leq a$ and $b'\leq b$ such that $x=a'\vee b'$.
Also, recall that an element $x$ of a join-semilattice is \emph{join-irreducible} if $x=a\vee b$ implies $x=a$ or $x=b$.  
In our setting, the distributivity property can be depicted as follows:
\[
\xymatrix@R=20pt@C=20pt{
	&\Cc_1\vee\Cc_2\ar@{..}[dl]\ar@{..}[dr]\ar@{..}[d]&&&&\Cc_1\vee\Cc_2\ar@{..}[dl]\ar@{..}[dr]\ar@{..}[d]&\\
	\Cc_1&\Dd&\Cc_2&\Longrightarrow&\Cc_1\ar@{..}[d]&\Dd=\Cc_1'\vee\Cc_2'\ar@{..}[dl]\ar@{..}[dr]&\Cc_2\ar@{..}[d]\\
	&&&&\Cc_1'&&\Cc_2'\\
}
\]


The next general easy lemma on covers in distributive join-semilattices will be useful.

\begin{lem}
	\label{lem:slcover}
	Let $(X,\leq)$ be a distributive join-semilattice (with join $\vee$). If $a\cover b$ and $b\not\leq a\vee c$, then $a\vee c\cover b\vee c$.
\end{lem}
\begin{proof}
	Assume $a\vee c\leq x\leq b\vee c$. As $(X,\leq)$ is distributive there exist $b'\leq b$ and $c'\leq c$ with $x=b'\vee c'$. Thus $a\leq a\vee b'\leq b$. As $a\cover b$, either $a=a\vee b'$ (thus $b'\leq a$) and thus $x=a\vee c$, or $a\vee b'=b$ and then $b\vee c\leq a\vee b'\vee c\leq a\vee x\vee c=x\leq b\vee c$ thus $x=b\vee c$. Hence either $a\vee c=b\vee c$ (which would contradict $b\not\leq a\vee c$), or $a\vee c\cover b\vee c$.
\end{proof}

In our setting, the statement of \Cref{lem:slcover} can be depicted as follows (where plain lines represent $\sqsubset$ and thick lines represent covers).

\begin{center}
	\includegraphics[width=.67\textwidth]{L21-11}
\end{center}


\section{The transduction semilattices $(\mathfrak C,\sqsubseteq_\FO^\circ)$ and $(\mathfrak C,\sqsubseteq_\FO)$}
%\todo[R2]{Unfortunately, I had to give up on most of this section. Wherever you can draw a picture, please do so. If you can make the structure of your proofs clearer with additional comments, please also do this.}
%\missingfigure{Anything to explain}
The aim of this section is to prove that $(\mathfrak C,\sqsubseteq_\FO^\circ)$ and $(\mathfrak C,\sqsubseteq_\FO)$ are distributive join-semilattices and to state some of their properties.

\begin{lem}
	\label{cl:union}
 If $\Dd\sqsubseteq\Cc_1\cup \Cc_2$, then there is a partition of $\Dd$ into $\Dd_1$ and $\Dd_2$ with $\Dd_1\sqsubseteq\Cc_1$ and 	$\Dd_2\sqsubseteq\Cc_2$.
 	If  $\Dd$ is additive, then
	$\Dd\sqsubseteq\Cc_1\cup \Cc_2\ \iff\ \Dd\sqsubseteq\Cc_1\text{ or }\Dd\sqsubseteq\Cc_2$.
\end{lem}
\begin{proof}
The first statement is straightforward.
We now prove the second statement.
%For an integer $n$, let $G_n$ be the disjoint union of all the graphs in $\Dd$ with at most $n$ vertices.
%As $\Dd$ is additive we have $G_n\in\Dd$. Assume $\Dd\sqsubseteq\Cc_1\union \Cc_2$. According to the first statement, there exists a partition $\Dd_1\union \Dd_2$ of $\Dd$ with
%	$\Dd_1\sqsubseteq\Cc_1$ and $\Dd_2\sqsubseteq\Cc_2$.
%	Let $i\in\{1,2\}$ be such that  $\Cc_i$ contains infinitely many graphs $G_n$.
%Then the generic (non-copying) transduction $\mathsf T$ allowing to extract an induced subgraph witnesses $\Cc\sqsubseteq\Cc_i$, thus $\Dd\sqsubseteq\Cc_i$. 

Assume $\Dd$ is additive and $\Dd\sqsubseteq\Cc_1\cup\Cc_2$.
According to the first statement, there exists a partition $\Dd_1,\Dd_2$ of $\Dd$ with 
$\Dd_1\sqsubseteq\Cc_1$ and $\Dd_2\sqsubseteq\Cc_2$.
For $G\in\Dd$ define \mbox{$\mathscr S(G)=\{H\union G: H\in\Dd\}$}. Note that $\mathscr S(G)\subseteq\Dd+\Dd$.
Let $\Dd'=\Dd+\Dd$. As $\Dd'\equiv \Dd\sqsubseteq\Dd_1\cup\Dd_2$ there exists a partition $\Dd_1',\Dd_2'$ of $\Dd'$ with $\Dd_1'\sqsubseteq\Dd_1$ and $\Dd_2'\sqsubseteq\Dd_2$.
If for every $G\in\Dd$ we have $\mathscr S(G)\cap \Dd_1'\neq\emptyset$, then $\Dd\sqsubseteq \Dd_1'$ (by the hereditary transduction), thus $\Dd\equiv\Dd_1\sqsubseteq\Cc_1$. 
Similarly, if for every $G\in\Cc$ we have $\mathscr S(G)\cap \Dd_2'\neq\emptyset$, then $\Dd\sqsubseteq\Cc_2$. Assume for contradiction that there exist $G_1,G_2\in\Dd$ with $\mathscr S(G_1)\cap \Dd_1'=\emptyset$ and $\mathscr S(G_2)\cap \Dd_2'=\emptyset$. Then $G_1\union G_2$ belongs neither to~$\Dd_1'$ nor to $\Dd_2'$, contradicting the assumption that $\Dd_1',\Dd_2'$ is a partition of $\Dd'=\Dd+\Dd$.
\end{proof}

\begin{lem}
\label{lem:irred1}
 If $\Cc_1$ and $\Cc_2$ are incomparable, then $\Cc_1\cup\Cc_2$ is not additive. 
  In particular, $\Cc_1\cup\Cc_2\not\equiv\Cc_1+\Cc_2$. 
 \end{lem}
 \begin{proof}
 	We prove by contradiction that $\Cc_1\cup\Cc_2$ is not  additive.
	Assume that we have $\Dd\sqsubseteq \Cc_1\cup\Cc_2$, where $\Dd$ is additive. According to \Cref{cl:union} we have $\Dd\sqsubseteq \Cc_1$ or $\Dd\sqsubseteq \Cc_2$, thus if $\Cc_1\cup\Cc_2\sqsubseteq\Dd$, then 
	$\Cc_2\sqsubseteq \Cc_1$ or $\Cc_1\sqsubseteq \Cc_2$, contradicting the hypothesis that $\Cc_1$ and $\Cc_2$ are incomparable.
 \end{proof}

\begin{thm}
\label{thm:sl}
	The quasi-order $(\mathfrak C,\sqsubseteq)$ is a distributive join-semilattice, where the join of $\Cc_1$ and $\Cc_2$ is $\Cc_1\cup\Cc_2$. In this quasi-order, additive classes are join-irreducible.
	This quasi-order has a minimum $\Ee$ and a maximum $\Gg$.
\end{thm}
\begin{proof}
	Of course we have $\Cc_1\sqsubseteq \Cc_1\cup\Cc_2$ and $\Cc_2\sqsubseteq \Cc_1\cup\Cc_2$. 
	Now assume $\Dd$ is such that $\Cc_1\sqsubseteq\Dd$ and  $\Cc_2\sqsubseteq\Dd$. 
	Let $\mathsf T_1$ and $\mathsf T_2$ be transductions encoding $\Cc_1$ and $\Cc_2$ in $\Dd$, with associated interpretations $\mathsf I_1=(\nu_1,\eta_1)$ and $\mathsf I_2=(\nu_1,\eta_1)$. 
	 By relabeling the colors, we can assume that the set ${\mathcal U}_1$ of unary relations used by $\mathsf I_1$ is disjoint from the set ${\mathcal U}_2$ of unary relations used by~$\mathsf I_2$. 
	 Without loss of generality, we have $\mathsf T_1=\mathsf I_1\circ\Gamma_{{\mathcal U}_1}\circ\mathsf C$ and 
	 $\mathsf T_2=\mathsf I_2\circ\Gamma_{{\mathcal U}_2}\circ\mathsf C$, where $\mathsf C$ is a copying operation if $\sqsubseteq$ is $\sqsubseteq_\FO$, or the identity mapping if $\sqsubseteq$ is $\sqsubseteq_\FO^\circ$.
	 Let $M$ be a new unary relation. We define the interpretation $\mathsf I=(\nu,\eta)$ by
	$\nu:=\big((\exists v\ M(v))\wedge \nu_1\big)\vee \big(\neg(\exists v\ M(v))\wedge \nu_2\big)$ and $\eta:=\big((\exists v\ M(v))\wedge \eta_1\big)\vee \big(\neg(\exists v\ M(v))\wedge \eta_2\big)$. Let $G\in\Cc_1\cup \Cc_2$. If $G\in\Cc_1$, then there exists a coloring $H^+$ of $H\in\mathsf C(\Dd)$ with $G=\mathsf I_1(H^+)$. We define~$H^*$ as the expansion of~$H^+$ where all vertices also belong to the unary relation~$M$. Then $G=\mathsf I(H^*)$. Otherwise, if $G\in\Cc_2$, then there exists a coloring $H^+$ of $H\in\mathsf C(\Dd)$ with $G=\mathsf I_2(H^+)$ thus
	$G=\mathsf I(H^+)$. As we did not introduce new copying transductions we deduce $\Cc_1\cup\Cc_2\sqsubseteq\Dd$.	
	It follows that~$(\mathfrak C,\sqsubseteq)$ is a join semi-lattice, which is distributive according to \Cref{cl:union}.
	
	That additive classes are join-irreducible follows from \Cref{lem:irred1}.
\end{proof}
Using the distributive join-semillatice structure of $(\mathfrak C,\sqsubseteq)$, the following corollaries follow directly from \Cref{lem:slcover}.
\begin{cor}
%\begin{lem}
\label{lem:cover}
 If $\Cc_1\cover\Cc_2$ and $\Cc_2\not\sqsubseteq\Cc_1\cup\Dd$, then $\Cc_1\cup\Dd\cover\Cc_2\cup\Dd$.
%\end{lem}
\end{cor}
%\begin{proof}
%		Let $\Ff$ be a class with 
%	$\Cc_1\union\Dd\sqsubseteq\Ff\sqsubseteq\Cc_2\union\Dd$.
%	According to \Cref{cl:union} there exists a partition $\Ff_1\union\Ff_2$ of $\Ff$ with $\Ff_1\sqsubseteq \Cc_2$ and $\Ff_2\sqsubseteq\Dd$. Thus $\Cc_1\sqsubseteq \Cc_1\union \Ff_1\sqsubseteq \Cc_2$.
%	As $\Cc_1\cover\Cc_2$ either $\Cc_1\equiv \Cc_1\union \Ff_1$ (i.e. $\Ff_1\sqsubseteq \Ff_1$)
% and thus $\Ff\equiv \Cc_1\union\Dd$ or $ \Cc_1\union \Ff_1\equiv \Cc_2$ 
%and then $\Cc_2\union\Dd\sqsubseteq \Cc_1\union \Ff_1\union \Dd\sqsubseteq  \Cc_1\union \Ff\union \Dd\equiv \Ff\sqsubseteq \Cc_2\union\Dd$ (i.e. $\Cc_2\union\Dd\equiv \Ff$). Hence $\Cc_1\union\Dd\equiv\Cc_2\union\Dd$ or $\Cc_1\union\Dd\cover\Cc_2\union\Dd$. The first case cannot happen as $\Cc_2\not\sqsubseteq \Cc_1\union \Dd$ by assumption.
%\end{proof}

\begin{cor}
\label{cor:corcover}
	If $\Cc_1\cover\Cc_2$, $\Cc_1\sqsubseteq\Dd$, and $\Cc_2$ and $\Dd$ are incomparable, then $\Dd\cover \Dd\cup\Cc_2$. 
\end{cor}
\begin{proof}
As $\Cc_2\not\sqsubseteq\Dd$ and $\Cc_1\sqsubseteq\Dd$ we have $\Cc_2\not\sqsubseteq \Dd\cup\Cc_1$.
\end{proof}
\begin{cor}
\label{cor:covR}
	If $\Cc_1\cover\Cc_2$, $\Cc_2$ and $\Dd$ are incomparable and $\Cc_2$ is additive, then $\Cc_1\cup\Dd\cover\Cc_2\cup\Dd$.
\end{cor}


\section{The transduction semilattices $(\mathfrak A,\sqsubseteq_\FO^\circ)$ and $(\mathfrak A,\sqsubseteq_\FO)$}
The aim of this section is to prove that $(\mathfrak A,\sqsubseteq_\FO^\circ)$ and $(\mathfrak A,\sqsubseteq_\FO)$ are distributive join-semilattices and to state some of their properties.

%\pom{
%\begin{lem}
%%\label{lem:irred2}
% If $\Cc_1$ and $\Cc_2$ are incomparable, then $\Cc_1+\Cc_2$ is not essentially connected.
% \end{lem}
%}
% \begin{proof}
%	We prove by contradiction that $\Cc_1+\Cc_2$ is not essentially connected.
%	It is immediate that ${\rm Conn}(\Cc_1+\Cc_2)\sqsubseteq\Cc_1\cup\Cc_2$. So if $\Cc_1+\Cc_2$ is essentially connected, then  $\Cc_1\cup \Cc_2$ and $\Cc_1+\Cc_2$ are equivalent, contradicting \Cref{lem:irred1}.
% \end{proof}



\begin{lem}
\label{lem:plus_sl}
A class $\Dd$ is additive if and only if 
	 for all classes $\Cc_1, \Cc_2$ we have
	\[
	\Cc_1+\Cc_2\sqsubseteq\Dd\qquad\iff\qquad\Cc_1\sqsubseteq\Dd\text{ and }\Cc_2\sqsubseteq\Dd.
\] 
\end{lem}
\begin{proof}
Assume $\Dd$ is additive.
	If $\Cc_1+\Cc_2\sqsubseteq\Dd$, then $\Cc_1\cup\Cc_2\sqsubseteq\Dd$ thus 
	$\Cc_1\sqsubseteq\Dd$ and $\Cc_2\sqsubseteq\Dd$. Conversely, assume 
		 $\Cc_1\sqsubseteq\Dd$ and $\Cc_2\sqsubseteq\Dd$.
		 Then, according to \Cref{fact:add_gluing}, $\Cc_1+\Cc_2\sqsubseteq\Dd$.
		 
%	Then $\Cc_1\cup \Cc_2\sqsubseteq\Dd$. Let $\mathsf T=\mathsf I\circ\Gamma_{\mathcal U}\circ\mathsf C$ be a transduction such that $\Cc_1\cup\Cc_2\subseteq\mathsf T(\Dd)$, where $\mathsf I=(M(x),\phi(x,y))$ with $M\in{\mathcal U}$, and where~$\mathsf C$ is either a copying operation if $\sqsubseteq$ is~$\sqsubseteq_\FO$, or the identity mapping if $\sqsubseteq$ is $\sqsubseteq_\FO^\circ$.
%	Let~${\mathcal U}'$ be the signature obtained from ${\mathcal U}$ by adding two unary predicates~$A(x)$ and~$B(x)$.
%	We define~$\phi_A(x,y)$ (resp.\ $\phi_B(x,y)$) by replacing in $\phi(x,y)$ the predicate $M$ by the predicate~$A$ (resp.\ by the predicate $B$). Let $\phi'(x,y)=\bigl(A(x)\wedge A(y)\wedge \phi_A(x,y)\bigr)\vee \bigl(B(x)\wedge B(y)\wedge\phi_B(x,y)\bigr)$, let $\mathsf I'=(A(x)\vee B(x),\phi'(x,y))$, and let $\mathsf T'=\mathsf I'\circ\Gamma_{{\mathcal U}'}\circ\mathsf C$. Then it is easily checked that $\Cc_1+\Cc_2\subseteq\mathsf T'(\Dd+\Dd)\sqsubseteq\Dd$.
%Conversely, a

Now assume that for all classes $\Cc_1, \Cc_2$ we have $\Cc_1+\Cc_2\sqsubseteq\Dd\ \iff\ \Cc_1\sqsubseteq\Dd\text{ and }\Cc_2\sqsubseteq\Dd$. Then (by choosing $\Cc_1=\Cc_2=\Dd$) we deduce $\Dd+\Dd\equiv\Dd$.
\end{proof}

\begin{lem}
\label{lem:distributive}
Assume $\Dd$ is additive and  $\Cc_1$ and $\Cc_2$ are incomparable.
If $\Dd\sqsubseteq\Cc_1+\Cc_2$, then there exist  classes $\Dd_1$ and $\Dd_2$ such that 
$\Dd\equiv\Dd_1+\Dd_2$, $\Dd_1\sqsubseteq\Cc_1$ and $\Dd_2\sqsubseteq\Cc_2$. Moreover, if~$\Cc_1$ and $\Cc_2$ are additive we can require that $\Dd_1$ and $\Dd_2$ are additive.
\end{lem}
\begin{proof}
 According to \Cref{crl:slunion} there exists a copy operation $\mathsf C$ (which reduces to the identity if $\sqsubseteq$ is~$\sqsubseteq_\FO^\circ$) and an immersive transduction $\mathsf T_{\rm imm}$ such that $\Dd\subseteq\mathsf T_{\rm imm}\circ\mathsf C(\Cc_1+\Cc_2)$. Let $\mathsf I$ be the interpretation part of $\mathsf T_{\rm imm}$.
	Let $G\in\Dd$ and let $H^+$ be a coloring of $H=\mathsf C(K)$, with $K\in\mathsf \Cc_1+\Cc_2$ and $G=\mathsf I(H^+)$.
	As $\mathsf T_{\rm imm}$ is immersive, each connected component of $G$ comes from a connected component of $H^+$, hence from a connected component of $K$. By grouping the connected components used in $K$ by their origin ($\Cc_1$ or $\Cc_2$) we get that $G$ is the disjoint union of $G_1\in \mathsf T_{\rm imm}\circ \mathsf C(K_1)$ and $G_2\in \mathsf T_{\rm imm}\circ \mathsf C(K_2)$, where $K_1\in\Cc_1$ and $K_2\in\Cc_2$. 
	So $\Dd\sqsubseteq\Dd_1+\Dd_2$, where $\Dd_1\sqsubseteq\Cc_1$ and $\Dd_2\sqsubseteq\Cc_2$.
	Moreover, as obviously $\Dd_1\sqsubseteq\Dd$ and $\Dd_2\sqsubseteq\Dd$ we derive from \Cref{lem:plus_sl} that we have $\Dd_1+\Dd_2\sqsubseteq\Dd$. Hence $\Dd\equiv\Dd_1+\Dd_2$.
	For $i=1,2$, if~$\Cc_i$ is additive, then we can assume that $\Dd_i$ is also additive.
		\end{proof}
%	\pom{
%\begin{cor}
%%\label{cor:ec}
%	If $\Dd$ is additive and essentially connected, then
%	\[
%	\Dd\sqsubseteq\Cc_1+\Cc_2\quad\iff\quad\Dd\sqsubseteq\Cc_1\text{ or }\Dd\sqsubseteq\Cc_2.
%	\]
%\end{cor}
%\begin{proof}
%	According to \Cref{lem:distributive} there exist $\Dd_1,\Dd_2$ with $\Dd\equiv\Dd_1+\Dd_2$, $\Dd_1\sqsubseteq\Cc_1$ and $\Dd_2\sqsubseteq\Cc_2$. However, as~$\Dd$ is essentially connected, $\Dd_1$ and $\Dd_2$ cannot be incomparable. Thus $\Dd\sqsubseteq\Cc_1$ or $\Dd\sqsubseteq\Cc_2$.
%\end{proof}
%}


\begin{thm}
\label{thm:slA}
	The quasi-order $(\mathfrak A,\sqsubseteq)$ is a distributive join-semilattice, where the join of~$\Cc_1$ and $\Cc_2$ is $\Cc_1+\Cc_2$. 
	%\pom{In this quasi-order, essentially connected (additive) classes are join-irreducible.} 	
	This quasi-order has a minimum $\Ee$ and a maximum $\Gg$.
\end{thm}
\begin{proof}
	That $(\mathfrak A,\sqsubseteq)$ is a  join-semilattice follows from \Cref{lem:plus_sl}; that it is distributive follows from \Cref{lem:distributive}.
	% \pom{The last statement follows from \Cref{lem:irred2}.}
\end{proof}

Although we were not able to express some nice non-trivial condition ensuring that an additive class is join-irreducible in $(\mathfrak A,\sqsubseteq)$, the following lemma is sufficient in many applications.
Recall that a class of graphs $\Cc$ has the \emph{joint embedding property} if, for every two graphs $G_1,G_2\in\Cc$ there is a graph $H\in\Cc$ having both $G_1$ and $G_2$ as induced subgraphs.
The joint embedding property can be expressed as a special  joint encoding property: a class~$\Cc$ has the joint embedding property if and only if
\[
	\forall G_1,G_2\in\Cc\quad\exists U\in\Cc\quad \{G_1,G_2\}\subseteq \mathsf H(U),
\]
where $\mathsf H$ is the hereditary transduction.

\begin{lem}
	\label{lem:addage}
	Let $\Dd^c$ be a class of connected graphs with the joint embedding property, and let $\Dd$ be the class of all graphs whose connected components all belong to $\Dd^c$.
	
	Then, for every two addable classes $\Cc_1$ and $\Cc_2$ we have
	\[
	\Dd\sqsubseteq\Cc_1+\Cc_2\quad\iff\quad\Dd\sqsubseteq\Cc_1\text{ or }\Dd\sqsubseteq\Cc_2.
	\]
\end{lem}
\begin{proof}
	The right to left implication being trivial, we only prove the left-to-right implication.
	
	According to \Cref{crl:slunion}, as $\Dd$ is addable, there is an immersive transduction $\mathsf T$ with $\Dd\subseteq \mathsf T(\Cc_1+\Cc_2)$. As $\mathsf T$ is immersive, we deduce
	$\Dd^c\subseteq \mathsf T(\Cc_1)\cup\mathsf T(\Cc_2)$.
	As $\Dd^c$ has the joint embedding property,
	there exists, for each integer $n$, a graph $G_n\in\Dd^c$ with the property that every graph in $\Dd^c$ with at most $n$ vertices is an induced subgraph of $G_n$. Let $i\in\{1,2\}$ be such that 
	$G_n\in\mathsf T(\Cc_i)$ infinitely often. Let $\mathsf T'=\mathsf H\circ\mathsf T$, where $\mathsf H$ is  the hereditary transduction. We have $\Dd^c\subseteq\mathsf T'(\Cc_i)$. As $\mathsf T'$ is immersive and $\Cc_i$ is addable, we deduce by \Cref{lem:imm_con} that $\Dd\subseteq\mathsf T'(\Cc_i)$. Hence, $\Dd\sqsubseteq \Cc_1$ or $\Dd\sqsubseteq \Cc_2$.
\end{proof}


%\begin{lem}
%\label{lem:join}
%
%
%\noindent For every three classes $\Cc_1, \Cc_2,\Dd$ we have
%\[
%	\Cc_1\cup\Cc_2\sqsubseteq\Dd\qquad\iff\quad\Cc_1\sqsubseteq\Dd\text{ and }\Cc_2\sqsubseteq\Dd.
%\]
%If, furthermore, $\Dd$ is additive, then 
%\[
%	\Cc_1+\Cc_2\sqsubseteq\Dd\qquad\iff\quad\Cc_1\sqsubseteq\Dd\text{ and }\Cc_2\sqsubseteq\Dd.
%\]
%
%It follows that the poset $(\mathfrak C,\sqsubseteq)$ is a distributive join semi-lattice, in which the join of $\Cc_1$ and $\Cc_2$ is $\Cc_1\cup\Cc_2$ and that the poset $(\mathfrak A,\sqsubseteq)$ is a distributive join semi-lattice, in which the join of $\Cc_1$ and $\Cc_2$ is $\Cc_1+\Cc_2$.
%\end{lem}
%
%\begin{proof}
%	Of course we have $\Cc_1\sqsubseteq \Cc_1\cup\Cc_2$ and $\Cc_2\sqsubseteq \Cc_1\cup\Cc_2$. Thus if 
%	$\Cc_1\cup\Cc_2\sqsubseteq\Dd$ then $\Cc_1\sqsubseteq\Dd$ and $\Cc_2\sqsubseteq\Dd$.
%	Now assume $\Dd$ is such that $\Cc_1\sqsubseteq\Dd$ and  $\Cc_2\sqsubseteq\Dd$. 
%	Let $\mathsf T_1$ and $\mathsf T_2$ be transductions encoding $\Cc_1$ and $\Cc_2$ in $\Dd$, with associated interpretations $\mathsf I_1=(\nu_1,\eta_1)$ and $\mathsf I_2=(\nu_1,\eta_1)$. 
%	 By relabeling the colors, we can assume that the set ${\mathcal U}_1$ of unary relations used by $\mathsf I_1$ is disjoint from the set ${\mathcal U}_2$ of unary relations used by $\mathsf I_2$. 
%	 Without loss of generality, we have $\mathsf T_1=\mathsf I_1\circ\Gamma_{{\mathcal U}_1}\circ\mathsf C$ and 
%	 $\mathsf T_2=\mathsf I_2\circ\Gamma_{{\mathcal U}_2}\circ\mathsf C$, where $\mathsf C$ is a copying operation if $\sqsubseteq$ is $\sqsubseteq_\FO$, or the identity mapping if $\sqsubseteq$ is $\sqsubseteq_\FO^\circ$.
%	 Let $M$ be a new unary relation. We define the interpretation $\mathsf I=(\nu,\eta)$ by
%	$\nu:=\big((\exists v\ M(v))\wedge \nu_1\big)\vee \big(\neg(\exists v\ M(v))\wedge \nu_2\big)$ and $\eta:=\big((\exists v\ M(v))\wedge \eta_1\big)\vee \big(\neg(\exists v\ M(v))\wedge \eta_2\big)$. Let $G\in\Cc_1\cup \Cc_2$. If $G\in\Cc_1$, then there exists a coloring $H^+$ of $H\in\mathsf C(\Dd)$ with $G=\mathsf I_1(H^+)$. We define~$H^*$ as the expansion of $H^+$ where all vertices also belong to the unary relation~$M$. Then $G=\mathsf I(H^*)$. Otherwise, if $G\in\Cc_2$ then there exists a coloring $H^+$ of $H\in\mathsf C(\Dd)$ with $G=\mathsf I_2(H^+)$ thus
%	$G=\mathsf I(H^+)$. As we did not introduce new copying transductions we deduce $\Cc_1\cup\Cc_2\sqsubseteq\Dd$.	
%	It follows that  $(\mathfrak C,\sqsubseteq)$ is a join semi-lattice, that is distributive according to \Cref{cl:union}.
%%	Last, assume $\Ff$ is a class with $\Cc\sqsubseteq_\FO \Ff$ and  $\Dd\sqsubseteq_\FO \Ff$. Then there is a copy operation~$\mathsf C$ and two non-copying transductions $\mathsf T_1$ and $\mathsf T_2$ such that $\mathsf T_1$ is a transduction encoding $\mathsf C(\Cc)$ in $\Ff$ and $\mathsf T_2$ is a transduction encoding $\mathsf C(\Dd)$ in $\Ff$. According to the previous case, there is a non-copying transduction $\mathsf T$ encoding $\mathsf C(\Cc)\cup \mathsf C(\Dd)=\mathsf C(\Cc\cup \Dd)$ in $\Ff$.
%	
%
%	Now assume that $\Dd$ is additive. If $\Cc_1+\Cc_2\sqsubseteq\Dd$ then $\Cc_1\cup\Cc_2\sqsubseteq\Dd$ thus 
%	$\Cc_1\sqsubseteq\Dd$ and $\Cc_2\sqsubseteq\Dd$. Conversely, assume 
%		 $\Cc_1\sqsubseteq\Dd$ and $\Cc_2\sqsubseteq\Dd$.
%	Then $\Cc_1\cup \Cc_2\sqsubseteq\Dd$. Let $\mathsf T=\mathsf I\circ\Gamma_{\mathcal U}\circ\mathsf C$ be a transduction such that $\Cc_1\cup\Cc_2\subseteq\mathsf T(\Dd)$, where $\mathsf I=(M(x),\phi(x,y))$ with $M\in{\mathcal U}$, and where $\mathsf C$ is either a copying operation if $\sqsubseteq$ is $\sqsubseteq_\FO$, or the identity mapping if $\sqsubseteq$ is $\sqsubseteq_\FO^\circ$.
%	Let ${\mathcal U}'$ be the signature obtained from ${\mathcal U}$ by adding two unary predicates $A(x)$ and $B(x)$.
%	We define $\phi_A(x,y)$ (resp. $\phi_B(x,y)$) by replacing in $\phi(x,y)$ the predicate $M$ by the predicate $A$ (resp. by the predicate $B$). Let $\phi'(x,y)=A(x)\wedge A(y)\wedge \phi_A(x,y)\vee B(x)\wedge B(y)\wedge\phi_B(x,y)$, let $\mathsf I'=(A(x)\vee B(x),\phi'(x,y))$, and let $\mathsf T=\mathsf I'\circ\Gamma_{{\mathcal U}'}\circ\mathsf C$. Then it is easily checked that $\Cc_1+\Cc_2\subseteq\mathsf T'(\Dd)$.
%		It follows that  $(\mathfrak A,\sqsubseteq)$ is a join semi-lattice, that is distributive according to \Cref{lem:distributive}. 
%\end{proof}



%Recall that a class $\Cc$ is \emph{join-irreducible} a class join semilattice if, for every pair $\Cc_1,\Cc_2$ with join $\Cc$, one of $\Cc_1$ and $\Cc_2$ is equivalent to $\Cc$.
%
%\begin{cor}
%\label{cor:conn}
%	If $\Cc_1$ and $\Cc_2$ are incomparable and additive, then $\Cc_1+\Cc_2$ is not essentially connected. 	
%	Consequently, essentially connected additive classes are join-irreducible in $(\mathfrak A,\sqsubseteq_\FO^\circ)$ and $(\mathfrak A,\sqsubseteq_\FO)$.
%\end{cor}
%\begin{proof}
%	It is immediate that ${\rm Conn}(\Cc_1+\Cc_2)\subseteq\Cc_1\cup\Cc_2$.
%	Thus the statement follows from the fact that $\Cc_1\cup \Cc_2$ and $\Cc_1+\Cc_2$ are not equivalent in $(\mathfrak A,\sqsubseteq_\FO^\circ)$ and $(\mathfrak A,\sqsubseteq_\FO)$.
%\end{proof}

%\pom{
%	\begin{cor}
%	Assume that $\Cc_1$ and $\Cc_2$ are incomparable and additive, $\Dd$ is additive and essentially connected, $\Cc_1\sqsubseteq\Dd$, and $\Cc_2\sqsubseteq\Dd$. Then we have
%\[
%\Cc_1\cup\Cc_2\sqsubset\Cc_1+\Cc_2\sqsubset\Dd.
%\]
%\end{cor}
%}
%\pom{
%\begin{cor}
%%\label{cor:incomp}
%	Assume that $\Cc_1$ and $\Cc_2$ are incomparable and additive, $\Dd$ is additive and essentially connected, $\Dd$ is incomparable with $\Cc_1$ and $\Cc_2\sqsubset\Dd$.
%	Then $\Cc_1+\Cc_2$ is incomparable with $\Dd$.
%\end{cor}
%}
%\begin{proof}
%	Assume for contradiction that $\Cc_1+\Cc_2\sqsubseteq\Dd$.
%	According to \Cref{thm:slA}, we have $\Cc_1\sqsubseteq\Dd$, contradicting the assumption that $\Dd$ is incomparable with $\Cc_1$.
%	
%	Assume for contradiction that $\Dd\sqsubseteq\Cc_1+\Cc_2$. 
%	According to \Cref{thm:slA} there exists (by distributivity) classes $\Dd_1$ and $\Dd_2$ with $\Dd_1\sqsubseteq\Cc_1$, $\Dd_2\sqsubseteq\Cc_2$, and $\Dd=\Dd_1+\Dd_2$. As $\Dd$ is essentially connected, according to \Cref{thm:slA} it is join-irreducible. Thus $\Dd_1$ and $\Dd_2$ are comparable. 
%	Thus  $\Dd\subseteq\Cc_1$ or $\Dd\subseteq\Cc_2$. The first case does not hold as $\Dd$ is incomparable with $\Cc_1$, and the second case does not hold as $\Cc_2\sqsubset\Dd$.
%\end{proof}

%\begin{cor}
%	We have $\Tt_2\cup\Pp\sqsubset_\FO\Tt_2+\Pp\sqsubset_\FO \PW_1$ and, for $n\geq 1$,
%	$\PW_n\cup\Tt_{n+2}\sqsubset_\FO \PW_n+\Tt_{n+2}\sqsubset_\FO\PW_{n+1}$.
%\end{cor}


%We now state a lemma, which give a sufficient condition for a cover to give rise, by taking the joins with a third class, to a new cover.
Using the distributive join-semillatice structure of $(\mathfrak A,\sqsubseteq)$, the following corollaries follow from \Cref{lem:slcover}.
\begin{cor}
%\begin{lem}
\label{lem:coverA}
 If $(\Cc_1,\Cc_2)$ is a cover in $(\mathfrak A,\sqsubseteq)$ and $\Cc_2\not\sqsubseteq\Cc_1+\Dd$  then $(\Cc_1+\Dd$, $\Cc_2+\Dd)$ is a cover in $(\mathfrak A,\sqsubseteq)$.
%\end{lem}
\end{cor}
%\todo[R1]{Rather say that $(\Cc_1,\Cc_2)$ is a cover  *in* $(\mathfrak A,\sqsubseteq)$ or *with respect to* $(\mathfrak A,\sqsubseteq)$. \Add}
%\begin{proof}
%Assume $\Ff$ is additive and $\Cc_1+\Dd\sqsubseteq\Ff\sqsubseteq\Cc_2+\Dd$. 
%According to \Cref{lem:distributive} there exist additive classes $\Ff_1$ and $\Ff_2$ with $\Ff\equiv\Ff_1+\Ff_2$, $\Ff_1\sqsubseteq\Cc_2$ and $\Ff_2\sqsubseteq\Dd$. Thus $\Cc_1\sqsubseteq \Cc_1+\Ff_1\sqsubseteq \Cc_2$.
%As $(\Cc_1,\Cc_2)$ is a cover in $(\mathfrak A,\sqsubseteq)$, either $\Cc_1\equiv \Cc_1+\Ff_1$ (i.e. $\Cc_1\equiv \Ff_1$)
% and thus $\Ff\equiv \Cc_1+\Dd$ or $ \Cc_1+\Ff_1\equiv \Cc_2$ 
%and then $\Cc_2+\Dd\sqsubseteq \Cc_1+\Ff_1+\Dd\sqsubseteq  \Cc_1+\Ff+\Dd\equiv \Ff\sqsubseteq \Cc_2+\Dd$ (i.e. $\Cc_2+\Dd\equiv \Ff$). Hence $\Cc_1+\Dd\equiv\Cc_2+\Dd$ or $\Cc_1+\Dd\cover\Cc_2+\Dd$. The first case cannot happen as $\Cc_2\not\sqsubseteq \Cc_1+\Dd$ by assumption.
%\end{proof}
\begin{cor}
\label{cor:corcoverA}
	If $(\Cc_1,\Cc_2)$ is a cover of $(\mathfrak A,\sqsubseteq)$, $\Cc_1\sqsubseteq\Dd$, and $\Cc_2$ and $\Dd$ are incomparable, then $(\Dd,\Dd+\Cc_2)$ is a cover of $(\mathfrak A,\sqsubseteq)$. 
\end{cor}
%\begin{proof}
%As $\Cc_2\not\subseteq\Dd$ and $\Cc_1\sqsubseteq\Dd$ we have $\Cc_2\not\sqsubseteq \Dd\cup\Cc_1$;
%as $\Cc_2$ is additive then $\Cc_2\not\sqsubseteq \Dd\cup\Cc_1$ implies $\Cc_2\not\sqsubseteq \Dd+\Cc_1$.
%\end{proof}
\begin{cor}
\label{cor:covRA}
	If $(\Cc_1,\Cc_2)$ is a cover of $(\mathfrak A,\sqsubseteq)$, $\Cc_2$ and $\Dd$ are incomparable, and $\Cc_2$ is essentially connected, then
	$(\Dd,\Dd+\Cc_2)$ is a cover of $(\mathfrak A,\sqsubseteq)$.
\end{cor}

\input{special}
\end{comment}
\input{extended-dual}

==> special.tex <==

\section{The transduction quasi-order around bounded treewidth and pathwidth}
\label{sec:special}
In many examples of combinatorial hierarchies (such as treewidth, pathwidth, \dots), it is clear that the hierarchy is strict in the containment order. However, due to the strength of transductions, this may not be the case in the transduction quasi-order. For example, \cite{TWW-factor} shows the twin-width hierarchy collapses to a finite level in the FO-transduction quasi-order. In this section, we prove that the pathwidth hierarchy is strict in $\sqsubseteq_\FO$, and more generally focus on the structure of the partial order in the region of classes with bounded treewidth.
%In this section we consider the  poset $(\mathfrak C,\sqsubseteq_\FO)$.
%\todo[R2]{(poset not defined)}
%We focus on the structure of the partial order in the region of classes with bounded treewidth.
A schematic view of the structure of $(\mathfrak C,\sqsubseteq_\FO)$ on classes with treewidth at most~$2$ is shown in~\Cref{fig:TW2a}.

Recall that % since {\MSO} collapses to {\FO} 
on colored trees of
bounded depth we have the following chain of covers \cite{Ganian2017}, where $\Tt_n$ denotes the class of  forests with height $n$.
\[\Ee\cover_\FO
\Tt_2\cover_\FO\Tt_3\cover_\FO\ldots.\] 
%\todo[R2]{Recall that -- reference? In the next sentence, please recall the definition of the classes.}
We first prove
that parallel to this chain we have a chain of covers
\[\Ee\cover_\FO\Pp\cover_\FO\Pp\cup\Tt_2\cover_\FO\Pp\cup\Tt_3\cover_\FO\dots\]
and for all $n\geq 1$ we have $\Tt_n\cover_\FO\Pp\cup\Tt_n$.

%\begin{restatable}{lemmax}{lemEE}
%%\begin{lem}
%\label{lem:Ee}
%	A class $\Cc$ is a transduction in $\Ee$ (or, equivalently, $\Cc\equiv_\FO\Ee$) if and only if $\Cc$ is a perturbation of a class whose members have uniformly bounded size connected components. Furthermore, a class $\Cc$ is a non-copying transduction in $\Ee$ if and only if $\Cc$ is a perturbation of $\Ee$.
%%\end{lem}
%\end{restatable}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%\begin{lem}
%	\label{lem:Ee}
%	A class $\Cc$ is a transduction in $\Ee$ (or, equivalently, $\Cc\equiv_\FO\Ee$) if and only if $\Cc$ is a perturbation of a class whose members have uniformly bounded size connected components. Furthermore, a class $\Cc$ is a non-copying transduction in $\Ee$ if and only if $\Cc$ is a perturbation of $\Ee$.
%\end{lem}
%\begin{proof}
%	Assume that $\Cc$ is a perturbation of a class $\Dd$ and that all graphs in $\Dd$ have connected components of size at most $n$. Then $\Dd$ can obviously be obtained from $\Ee$ by the composition of an $n$-copy transduction composed with some (immersive) transduction. 
%	Conversely, if $\Cc$ is a transduction of $\Ee$ then, according to \Cref{thm:normal}, $\Cc$ is a perturbation of a class $\Dd\subseteq\mathsf T_{\rm imm}\circ \mathsf C(\Ee)$, where $\mathsf T_{\rm imm}$ is immersive and $\mathsf C$ is a $k$-copy transduction for some number $k$. By the strong locality of the interpretation associated to $\mathsf T_{\rm imm}$ no connected component of a graph in $\Dd$ can have size greater than $k$.
%	The last statement is obvious, as every immersive transduction of $\Ee$ is included in $\Ee$.
%\end{proof}
%%%%%%
%\begin{restatable}[\blah]{thm}{covers}
\begin{thm}
	\label{thm:covers}
	We have $\Ee\cover_\FO\Pp$ and, for every $n\geq 1$, the chain of covers
	%The following classes form a chain of
	%covers
	%\[\Ee\cover_\FO\Pp\cover_\FO\Pp\cup\Tt_2\cover_\FO\Pp\cup\Tt_3\cover_\FO\dots\]
	\[(\Pp+\Tt_n)\cover_\FO (\Pp+\Tt_n)\cup\Tt_{n+1}\cover_\FO(\Pp+\Tt_n)\cup\Tt_{n+2}\cover_\FO\dots\]
	In particular, for $n=1$ we get
	$\Pp\cover_\FO \Pp\cup\Tt_{2}\cover_\FO\Pp\cup\Tt_{3}\cover_\FO\dots$
	
	\noindent Moreover, for all $n\geq 1$ we have $\Tt_n\cover_\FO\Pp\cup\Tt_n$.
\end{thm}
%\end{restatable}
%%%%%%%%%%%%%%%%%%%%%
%\covers*
\begin{proof}
	Obviously $\Ee\sqsubset_\FO\Pp$. Assume towards a contradiction that 
	there exists a class $\Cc$ with \mbox{$\Ee\sqsubset_\FO\Cc\sqsubset_\FO\Pp$}.
	As in the first part of the proof of \Cref{thm:transpath}, we see that 
	the class~$\Cc$ is a perturbation of a class $\Dd$ with bounded bandwidth.  
	The connected components of the graphs in $\Dd$ have unbounded size as otherwise $\Dd$ (and thus $\Cc$) can be transduced in~$\Ee$ (according to \Cref{lem:Ee}). 
	But then $\Cc\equiv_\FO \Pp$ by \Cref{thm:transpath}, 
	contradicting our assumption. 
	Hence~$\Ee\cover_\FO\Pp$. 
	
	Let $m\geq n\geq 1$. We have $(\Pp+\Tt_n)\not\sqsubseteq_\FO\Tt_{m+1}$ and 
	$\Tt_{m+1}\not\sqsubseteq_\FO(\Pp+\Tt_n)\cup\Tt_m$ as otherwise, according to \Cref{cl:union} we would have $\Tt_{m+1}\sqsubseteq_\FO\Pp+\Tt_n$ or $\Tt_{m+1}\sqsubseteq_\FO\Tt_m$ as $\Tt_{m+1}$ is additive. 
	Let $\Pp'\equiv_\FO\Pp$ be the class of all linear forests and let 
	$\Yy_{m+1}$ be the class of all trees with height $m+1$.
	Note that $\Tt_{m+1}$ is the class of all graphs whose connected components all beglong to $\Yy_{m+1}$ and that $\Yy_{m+1}$ has the joint embedding property.
	As classes $\Pp'$, and $\Tt_n$ are addable,  according to \Cref{lem:addage},  we have that $\Tt_{m+1}\sqsubseteq_\FO\Pp+\Tt_n$ would imply  $\Tt_{m+1}\sqsubseteq_\FO\Pp$ or $\Tt_{m+1}\sqsubseteq_\FO\Tt_n$ (as $\Pp \equiv_\FO\Pp'$).
	Hence, $\Tt_{m+1}\not\sqsubseteq_\FO\Pp+\Tt_n$.
	According to \Cref{lem:cover} we have 	$(\Pp+\Tt_n)\cup\Tt_m\cover_\FO(\Pp+\Tt_n)\cup\Tt_{m+1}$. (Note that $\Tt_1=\Ee$ and thus $\Pp\cup\Tt_1=\Pp$, and that $(\Pp+\Tt_n)\cup\Tt_n=\Pp+\Tt_n$.)
	
	Let $n\geq 1$.
	According to \Cref{cor:corcover}, as $\Ee\cover_\FO\Pp$,  $\Ee\sqsubseteq_\FO\Tt_n$, and $\Pp$ is incomparable with $\Tt_n$ we have $\Tt_n\cover_\FO\Pp\cup\Tt_n$. 
\end{proof}
%%%%%%%%%%%%%%%%%%%%%
%\begin{proof}
%Obviously $\Ee\sqsubset_\FO\Pp$. Assume towards a contradiction that 
%there exists a class $\Cc$ with $\Ee\sqsubset_\FO\Cc\sqsubset_\FO\Pp$.
%As in the first part of the proof of \Cref{thm:transpath}, we see that 
%the class~$\Cc$ is a perturbation of a class $\Dd$ with bounded bandwidth.  
%The connected components of the graphs in $\Dd$ have unbounded size as otherwise $\Dd$ (and thus $\Cc$) can be transduced in $\Ee$ (according to \Cref{lem:Ee}). 
% But then $\Cc\equiv_\FO \Pp$ by \Cref{thm:transpath}, 
%contradicting our assumption. 
% Hence~$\Ee\cover_\FO\Pp$. 
% 
%		Let $m\geq n\geq 1$. We have $(\Pp+\Tt_n)\not\sqsubseteq_\FO\Tt_{m+1}$ and 
%		$\Tt_{m+1}\not\sqsubseteq_\FO(\Pp+\Tt_n)\cup\Tt_m$ as otherwise, according to \Cref{cl:union} we would have $\Tt_{m+1}\sqsubseteq_\FO\Pp+\Tt_n$ or $\Tt_{m+1}\sqsubseteq_\FO\Tt_m$ as $\Tt_{m+1}$ is additive. As $\Tt_{m+1}$ is additive and essentially connected $\Tt_{m+1}\sqsubseteq_\FO\Pp+\Tt_n$ would imply $\Tt_{m+1}\sqsubseteq_\FO\Pp$ or $\Tt_{m+1}\sqsubseteq_\FO\Tt_n$.
%		According to \Cref{lem:cover} we have 	$(\Pp+\Tt_n)\cup\Tt_m\cover_\FO(\Pp+\Tt_n)\cup\Tt_{m+1}$. (Note that $\Tt_1=\Ee$ and thus $\Pp\cup\Tt_1=\Pp$, and that $(\Pp+\Tt_n)\cup\Tt_n=\Pp+\Tt_n$.)
%		
%Let $n\geq 1$.
%		According to \Cref{cor:corcover}, as $\Ee\cover_\FO\Pp$,  $\Ee\sqsubseteq_\FO\Tt_n$, and $\Pp$ is incomparable with $\Tt_n$ we have $\Tt_n\cover_\FO\Pp\cup\Tt_n$. 
%\end{proof}

%\begin{lem}
%\label{lem:covunion_add}
%	Let $\Cc_1,\Cc_2,\Dd$ be additive classes.
%	If $(\Cc_1,\Cc_2)$ is a cover on additive classes and $\Dd$ is incomparable with $\Cc_2$ then 
%	$(\Cc_1+\Dd,\Cc_2+\Dd)$ is a cover on additive classes.
%\end{lem}
%\begin{proof}
%	First notice that $\Cc_1+\Dd\not\equiv_\FO\Cc_2+\Dd$ as otherwise, according to \Cref{lem:plus} we have
%	$\Cc_2\sqsubseteq_\FO\Cc_1+\Dd$ hence (by \Cref{fact:union}) $\Cc_2\sqsubseteq_\FO\Dd$, contradicting the assumption that $\Dd$ is incomparable with $\Cc_2$.
%	
%	Assume $\Ff$ is additive and $\Cc_1+\Dd\sqsubseteq_\FO\Ff\sqsubseteq_\FO\Cc_2+\Dd$. 
%	Then either $\Ff\equiv_\FO\Cc_2+\Dd$ or (by \Cref{lem:plus}) we have $\Ff\sqsubseteq_\FO\Cc_2\cup\Dd$.
%	According to \Cref{fact:union} we have $\Ff\sqsubseteq_\FO \Cc_2$ or $\Ff\sqsubseteq_\FO D$.
%	In the first case we get $\Cc_1+\Dd\sqsubseteq_FO \Cc_2$ hence (by \Cref{lem:plus}) 
%	$\Dd\sqsubseteq_\FO \Cc_2$, contradicting the assumption that $\Dd$ is incomparable with $\Cc_2$.
%	 In the latter case
%	we get $\Ff\sqsubseteq_\FO \Cc_1+\Ff\sqsubseteq_\FO \Cc_1+\Dd\sqsubseteq_\FO\Ff$ hence $\Ff\equiv_\FO\Cc_1+\Dd$.
%\end{proof}

%\begin{remark}
%  It is easy to check the following properties:
%  \begin{align*}
	%    \join M_1\join M_2&=\join M_2\join M_1,\\
	%    \join M\join M&=\mathsf{Id},
	%  \end{align*}
%  where $\mathsf{Id}$ denotes the identity transduction.
%\end{remark}


%%%%%%%%%%%%%%%%%%%%%%%
%\begin{enumerate}
%	\item $\PW_2\not\sqsubseteq_\FO\Tt$ (Lemma~\ref{lem:T-PW2});
% 	\item $\Tt\sqsubset_\FO \TW_2$ ($\TW_2\not\sqsubseteq_\FO \Tt$ follows from $\PW_2\not\sqsubseteq_\FO\Tt$);
% 	\item there is no class between the classes $\Tt_n$ and the class $\Tt$ (Lemma~\ref{lem:Tn-T});
% 	\item there is no class between $\Tt_n$ and $\Tt_{n+1}$ (by \cite{blumensath10} and \cite{Ganian2012}).
%	\item $\Pp\not\sqsubseteq_\FO \Tt_{n+1}\not\sqsubseteq_\FO\PW_n$ (the first was noticed in \cite{Ganian2012}; the second is proved in Lemma~\ref{lem:Tn-PW});
%	\item $\PW_n\sqsubset_\FO \PW_{n+1}$ (this follows from $\Tt_{n+1}\not\sqsubseteq_\FO\PW_n$ as  $\Tt_{n+1}\sqsubseteq_\FO\PW_{n+1}$).
%	\item $\Tt_n\sqsubset_\FO\PW_n$ (this follows from $\Tt_n$ non comparable with $\Pp$ and $\PW_n\supseteq \Tt_n\cup\Pp$);
%	\item $\PW_n$ non comparable with $\Tt$ (this follows from $\Tt_{n+1}\not\sqsubseteq_\FO \PW_n$ and $\PW_2\not\sqsubseteq_\FO\Tt$);
%	\item $\PW_n\sqsubset_\FO\TW_n$ (this follows from $\PW_n$ non comparable with $\Tt$ and $\TW_n\supseteq\PW_n\cup\Tt$);
%	\item $\BT\sqsubset_\FO\Tt$, where $\BT$ is the class of cubic trees;
%	\item Binary trees and Grids are non-comparable (Lemma~\ref{lem:GridBT});
%\end{enumerate}
%
%This section is devoted to the proof of \Crefrange{thm:covers}{thm:PWTW}, 
%shedding light on the parts of the transduction quasiorder involving forests with 
%bounded depth, paths, classes with bounded pathwidth, trees, and classes with bounded treewidth.  
%We recall the theorems for convenience. \Cref{thm:covers} follows basically from 
%our characterization of the equivalence class of the class of paths. 
%



%\covers*
%
%\begin{proof}
%Obviously $\Ee\sqsubset_\FO\Pp$. Assume towards a contradiction that 
%there exists a class $\Cc$ with $\Ee\sqsubset_\FO\Cc\sqsubset_\FO\Pp$.
%As in the first part of the proof of \Cref{thm:transpath}, we see that 
%the class~$\Cc$ is a perturbation of a class $\Dd$ with bounded bandwidth.  
%The connected components of the graphs in $\Dd$ have unbounded size as otherwise $\Dd$ (and thus $\Cc$) can be transduced in $\Ee$ (according to \Cref{lem:Ee}). 
% But then $\Cc\equiv_\FO \Pp$ by \Cref{thm:transpath}, 
%contradicting our assumption. 
% Hence~$\Ee\cover_\FO\Pp$. 
% 
%		Let $n\geq 1$.
%		According to \Cref{cor:corcover}, as $\Pp$ is incomparable with $\Tt_n$ and $\Ee\sqsubseteq_\FO\Tt_n$, we have 	$\Tt_n\cover_\FO\Pp\cup\Tt_n$. 
%		As $\Tt_n\cover_\FO\Tt_{n+1}$, $\Tt_{n+1}$ and $\Pp$ are incomparable and $\Tt_{n+1}$ is additive we deduce from \Cref{cor:covR} that $\Tt_n\cup\Pp\cover_\FO\Tt_{n+1}\cup\Pp$.
%\end{proof}

Let $\PW_n$ denote the class of all graphs with pathwidth at most $n$.
The difficult part of the next theorem is to prove that $\Tt_{n+2}\not\sqsubseteq_\FO\PW_n$. We use that the
class $\Tt_{n+2}$ is addable, which by \Cref{crl:slunion}
implies that we can eliminate perturbations and focus on immersive
transductions.
This allows us to consider host graphs in $\PW_n$ that have
bounded radius, where we can find a small set of vertices whose
removal decreases the pathwidth. We encode the adjacency 
to these vertices by colors and proceed by induction. 
%%%%%%%%%%%%%%%%%%%%%%%
%%
%
%Recall that a {\em star coloring} of a graph $G$ is  a proper coloring of $V(G)$ such that any two color classes induce a star forest (or, equivalently, such that no path of length four is $2$-colored), and that the the star chromatic number $\chi_{\rm st}(G)$ of $G$ is the minimum number of colors in a star coloring of $G$~\cite{alon2}. The star chromatic number is bounded on classes of graphs excluding a minor~\cite{Taxi_jcolor} and, more generally, on every bounded expansion class~\cite{nevsetvril2008grad}.
%
%\input{monotone}

%\begin{restatable}[\blah]{thm}{thmPW}
\begin{thm}
	\label{thm:PW}
	For $n\geq 1$ we have $\Tt_{n+1}\sqsubset_\FO\PW_n$ but
	\mbox{$\Tt_{n+2}\not\sqsubseteq_\FO\PW_n$}.
	%  Consequently, $\PW_n\cover_\FO \PW_n\cup \Tt_{n+2}\sqsubset_\FO \PW_n+\Tt_{n+2}\sqsubset_\FO \PW_{n+1}$.
	Consequently, for $m>n\geq 1$ we have
	
	\begin{align*}
		\Tt_m+\PW_n\cover_\FO (\Tt_m+\PW_n)\cup \Tt_{m+1}
		&  \cover_\FO (\Tt_m+\PW_n)\cup \Tt_{m+2}\cover_\FO \dots\\
		\Tt_m+\PW_n\cover_\FO (\Tt_m+\PW_n)\cup \Tt_{m+1}&\sqsubset_\FO\Tt_{m+1}+\PW_n.
	\end{align*}
	In particular, fixing $m=n+1$ we get that for $n\geq 1$ we have
	\begin{align*}
		\PW_n\cover_\FO \PW_n\cup \Tt_{n+2}&\cover_\FO \PW_n\cup \Tt_{n+3}\cover_\FO \dots\sqsubset_\FO\PW_{n}\cup\Tt\\
		\PW_n\cover_\FO \PW_n\cup \Tt_{n+2}&\sqsubset_\FO\Tt_{n+2}+\PW_n\sqsubset_\FO\PW_{n+1}.
	\end{align*}
\end{thm}
%\end{restatable}


%\thmPW*
\begin{proof}
	For convenience, we define $\Tt_1=\PW_0=\Ee$, which is consistent with our definitions.
	Then $\Tt_{n}\sqsubseteq_\FO\PW_{n-1}$ as for $n=1$ this reduces to $\Ee\sqsubseteq_\FO\Ee$ and, if $n>1$, $\Tt_{n}\sqsubset_\FO\Pp\cup \Tt_{n}\subset \PW_{n-1}$. We now prove $\Tt_{n+1}\not\sqsubseteq_\FO\PW_{n-1}$
	by induction on $n$. For $n=1$, this follows from \Cref{lem:Ee} (or from the known fact $\Tt_2\sqsupset\Ee$). 
	Now assume that we have proved the statement for~$n\geq 1$ and assume towards a contradiction that $\Tt_{n+2}\sqsubseteq_\FO\PW_{n}$.
	The class~$\PW_{n}$ is the monotone closure of the class $\mathcal{I}_{n+1}$ of interval graphs with clique number at most~$n+1$. As the class~$\mathcal{I}_{n+1}$ has bounded star chromatic number, it follows from \Cref{lem:monotone} that $\PW_{n}\sqsubseteq_\FO\mathcal{I}_{n+1}$. Let~$\mathsf T$ be the composition of the respective transductions, so that  $\Tt_{n+2}\subseteq\mathsf T(\mathcal{I}_{n+1})$.
	As $\Tt_{n+3}$ is additive, 
	it follows from \Cref{crl:slunion} that there is a copy operation $\mathsf C$ and an immersive transduction~$\mathsf{T}_0$ such that $\mathsf T_0\circ \mathsf C$ subsumes~$\mathsf T$.
	As $\{G+K_1: G\in\Tt_{n+1}\}\subseteq \Tt_{n+2}$ if follows from \Cref{cor:apex} that there exists an integer~$r$ such that $\Tt_{n+1}\sqsubseteq^\circ_\FO \rloc{r}{\mathsf C(\mathcal I_{n+1})}\subseteq \mathsf C(\rloc{r}{\mathcal I_{n+1}})$. According to \Cref{lem:slunion}, as $\Tt_{n+1}$ is additive, there exists an immersive transduction $\mathsf{T}_1$ with $\Tt_{n+1}\subseteq \mathsf T_1\circ\mathsf C(\rloc{r}{\mathcal I_{n+1}})$.
	
	Let $G\in \rloc{r}{\mathcal I_{n+1}}$ and let $P$ be a shortest path connecting the 
	minimal and maximal vertices in an interval representation of $G$. Then $P$ has length at most $2r$, $P$ dominates $G$, and  $G-P\in\mathcal I_n$. 
	By encoding the adjacencies in~$G$ to the vertices of $P$ by a monadic expansion, we get that that there exists a transduction~$\mathsf T_2$ (independent of our choice of $G$) such that $G$ is a $\mathsf T_2$-transduction of $H$, where $H$ is obtained from $G$ by deleting all the edges incident to a  vertex in $P$. 
	In particular, $\rloc{r}{\mathcal I_{n+1}}\subseteq\mathsf T_2(\mathcal I_n)$ thus
	$\Tt_{n+1}\subseteq\mathsf T_1\circ\mathsf C\circ\mathsf T_2(\mathcal I_n)$, which contradicts our induction hypothesis. 
	
	
	Let us now prove the cover chain, that is, for $k\geq m>n\geq 1$ we have
	\mbox{$(\Tt_m+\PW_n)\cup\Tt_k$} $\cover_\FO (\Tt_m+\PW_n)\cup \Tt_{k+1}$. To deduce this from the cover
	$\Tt_k\cover_\FO\Tt_{k+1}$ using \Cref{lem:cover} we need to check
	$(\Tt_m+\PW_n)\not\sqsubseteq_\FO \Tt_{k+1}\not\sqsubseteq_\FO (\Tt_m+\PW_n)\cup\Tt_k$.
	According to \Cref{lem:plus_sl}, as $(\Tt_m+\PW_n)$ and $\Tt_{k+1}$ are both additive,
	$(\Tt_m+\PW_n)\sqsubseteq_\FO \Tt_{k+1}$ is equivalent to $\Tt_m\sqsubseteq_\FO  \Tt_{k+1}$  and
	$\PW_n\sqsubseteq_\FO  \Tt_{k+1}$. However, $\PW_n\not\sqsubseteq_\FO  \Tt_{k+1}$ as $\Pp\sqsubseteq_\FO\PW_n$ and $\Pp$ is incomparable with $\Tt_{k+1}$. Thus $(\Tt_m+\PW_n)\not\sqsubseteq_\FO \Tt_{k+1}$.
	Now assume for contradiction that we have $\Tt_{k+1}\sqsubseteq_\FO (\Tt_m+\PW_n)\cup\Tt_k$.
	As $\Tt_{k+1}$ is additive, it follows from \Cref{cl:union} that we have
	$\Tt_{k+1}\sqsubseteq_\FO (\Tt_m+\PW_n)$ (as $\Tt_{k+1}\not\sqsubseteq_\FO \Tt_k$).
	According to \Cref{lem:addage},  $\Tt_{k+1}\sqsubseteq_\FO \Tt_m$ or $\Tt_{k+1}\sqsubseteq_\FO\PW_n$. 
The first case does not hold as $k+1>m$. The second case does not hold as $k+1\geq n+2$ and $\Tt_{n+2}\not\sqsubseteq_\FO\PW_n$.
\end{proof}
\begin{cor}
\label{cor:PWTW}
For $n\geq 1$ we have $\PW_n\sqsubset_\FO\TW_n$.
\end{cor}
\begin{proof}
	As $\PW_n$ is included in $\TW_n$ we have $\PW_n\sqsubseteq_\FO\TW_n$.
According to \Cref{thm:PW} we have
$\Tt_{n+2}\not\sqsubset_\FO\PW_n$. As $\Tt_{n+2}$ is included in 
$\TW_n$, we deduce $\TW_{n}\not\sqsubset_\FO\PW_n$.
\end{proof}	

%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{proof}
%For convenience, we define $\Tt_1=\PW_0=\Ee$, which is consistent with our definitions.
%Then $\Tt_{n}\sqsubseteq_\FO\PW_{n-1}$ as for $n=1$ this reduces to $\Ee\sqsubseteq_\FO\Ee$ and, if $n>1$, $\Tt_{n}\sqsubset_\FO\Pp\cup \Tt_{n}\subset \PW_{n-1}$. We now prove $\Tt_{n+1}\not\sqsubseteq_\FO\PW_{n-1}$
%		 by induction on $n$. For $n=1$, this follows from \Cref{lem:Ee} (or from the known fact $\Tt_2\sqsupset\Ee$). 
%		 Now assume that we have proved the statement for~$n\geq 1$ and assume towards a contradiction that $\Tt_{n+2}\sqsubseteq_\FO\PW_{n}$.
%		The class~$\PW_{n}$ is the monotone closure of the class $\mathcal{I}_{n+1}$ of interval graphs with clique number at most~$n+1$. As the class~$\mathcal{I}_{n+1}$ has bounded star chromatic number, it follows from \Cref{lem:monotone} that $\PW_{n}\sqsubseteq_\FO\mathcal{I}_{n+1}$. Let~$\mathsf T$ be the composition of the respective transductions, so that  $\Tt_{n+2}\subseteq\mathsf T(\mathcal{I}_{n+1})$.
%		As $\Tt_{n+3}$ is additive, 
%		it follows from \Cref{crl:slunion} that there is a copy operation $\mathsf C$ and an immersive transduction $\mathsf{T}_0$ such that $\mathsf T_0\circ \mathsf C$ subsumes $\mathsf T$.
%		As $\{G+K_1: G\in\Tt_{n+1}\}\subseteq \Tt_{n+2}$ if follows from \Cref{cor:apex} that there exists an integer $r$ such that $\Tt_{n+1}\sqsubseteq^\circ_\FO \rloc{r}{\mathsf C(\mathcal I_{n+1})}\subseteq \mathsf C(\rloc{r}{\mathcal I_{n+1}})$. According to \Cref{lem:slunion}, as $\Tt_{n+1}$ is additive, there exists an immersive transduction $\mathsf{T}_1$ with $\Tt_{n+1}\subseteq \mathsf T_1\circ\mathsf C(\rloc{r}{\mathcal I_{n+1}})$.
%		
%		Let $G\in \rloc{r}{\mathcal I_{n+1}}$ and let $P$ be a shortest path connecting the 
%minimal and maximal vertices in an interval representation of $G$. Then $P$ has length at most $2r$, $P$ dominates $G$, and  $G-P\in\mathcal I_n$. 
%		By encoding the adjacencies in~$G$ to the vertices of $P$ by a monadic expansion, we get that that there exists a transduction~$\mathsf T_2$ (independent of our choice of $G$) such that $G$ is a $\mathsf T_2$-transduction of $H$, where $H$ is obtained from $G$ by deleting all the edges incident to a  vertex in $P$. 
%		In particular, $\rloc{r}{\mathcal I_{n+1}}\subseteq\mathsf T_2(\mathcal I_n)$ thus
%		$\Tt_{n+1}\subseteq\mathsf T_1\circ\mathsf C\circ\mathsf T_2(\mathcal I_n)$, which contradicts our induction hypothesis. 
%
%
%Let us now prove the cover chain, that is that for $k\geq m>n\geq 1$ we have
%$(\Tt_m+\PW_n)\cup\Tt_k\cover_\FO (\Tt_m+\PW_n)\cup \Tt_{k+1}$. To deduce this from the cover
%$\Tt_k\cover_\FO\Tt_{k+1}$ using \Cref{lem:cover} we need to check
%$(\Tt_m+\PW_n)\not\sqsubseteq_\FO \Tt_{k+1}\not\sqsubseteq_\FO (\Tt_m+\PW_n)\cup\Tt_k$.
%According to \Cref{lem:join}, as $(\Tt_m+\PW_n)$ and $\Tt_{k+1}$ are both additive,
%$(\Tt_m+\PW_n)\sqsubseteq_\FO \Tt_{k+1}$ is equivalent to $\Tt_m\sqsubseteq_\FO  \Tt_{k+1}$  and
%$\PW_n\sqsubseteq_\FO  \Tt_{k+1}$. However, $\PW_n\not\sqsubseteq_\FO  \Tt_{k+1}$ as $\Pp\sqsubseteq_\FO\PW_n$ and $\Pp$ is incomparable with $\Tt_{k+1}$. Thus $(\Tt_m+\PW_n)\not\sqsubseteq_\FO \Tt_{k+1}$.
%Now assume for contradiction that we have $\Tt_{k+1}\sqsubseteq_\FO (\Tt_m+\PW_n)\cup\Tt_k$.
%As $\Tt_{k+1}$ is additive, it follows from \Cref{cl:union} that we have
%$\Tt_{k+1}\sqsubseteq_\FO (\Tt_m+\PW_n)$ (as $\Tt_{k+1}\not\sqsubseteq_\FO Tt_k$).
%As $\Tt_{k+1}$ is additive and essentially connected, according to \Cref{cor:ec} we deduce that  $\Tt_{k+1}\sqsubseteq_\FO \Tt_m$ or $\Tt_{k+1}\sqsubseteq_\FO\PW_n$. The first case does not hold as $k+1>m$. The second case does not hold as $k+1\geq n+2$ and $\Tt_{n+2}\not\sqsubseteq_\FO\PW_n$.
%\end{proof}

%Again, \Cref{crl:slunion} brings us quickly to the result of \Cref{thm:PWTW}. 
%%%%%%%%%%%%%%%
%\begin{restatable}[\blah]{thm}{PWTW}



\begin{thm}
	\label{thm:PWTW}
	For $m>n\geq 2$ , $\Tt_m+\PW_n$ is incomparable with~$\Tt$.
	Consequently, we have 
	\[\Tt\sqsubset_\FO\Tt\cup\PW_2\sqsubset_\FO\Tt\cup(\Tt_4+\PW_2)\sqsubset_\FO\dots\sqsubset_\FO\Tt+\PW_2\sqsubset_\FO\TW_2.\]
\end{thm}
%\end{restatable}
%\PWTW*
\begin{proof}
	We establish that $\PW_2\not\sqsubseteq_\FO\Tt$, from which $\TW_2\not\sqsubseteq_\FO \Tt$ immediately follows.
	Assume for contradiction that $\PW_2\sqsubseteq_\FO\Tt$. 
	As $\PW_2$ is additive and \dnnc (Fact~\ref{fact:non-copy-classes}), by \Cref{crl:slunion} there is an immersive transduction of $\PW_2$ in $\Tt$. In particular, there exists an integer $r$ such that the class $\{K_1\join P_n: n\in\mathbb N\}$ is the transduction of $\Tt_r$, which contradicts the property 
	$\Pp\not\sqsubseteq_\FO\Tt_r$. Thus  $\PW_2\not\sqsubseteq_\FO\Tt$.
	
	
	
	We prove that the classes $\PW_n$ ($n\geq 2$) are incomparable with $\Tt$.
	The class $\Tt$ has unbounded linear cliquewidth, hence $\Tt\not\sqsubseteq_\FO\Hh$, and thus \mbox{$\Tt\not\sqsubseteq_\FO\PW_n$} for every integer~$n$ (recall that a class $\Cc$ has bounded linear cliquewidth if and only if $\Cc\sqsubseteq_\FO \Hh$). As $\PW_2\not\sqsubseteq_\FO\Tt$ it follows that,  for $n\geq 2$,  $\PW_n\not\sqsubseteq_\FO\Tt$, thus $\PW_n$ and~$\Tt$ are incomparable. 
	(This settles the case where $m=n+1$ as $\Tt_{n+1}+\PW_n=\PW_n$.)
	For $m>n+1$ the classes $\Tt_m$ and $\PW_n$ are additive and incomparable and $\Tt_m\sqsubset_\FO\Tt$.
	Then, it follows from \Cref{lem:addage} that  $\Tt\not\sqsubseteq_\FO\Tt_m+\PW_n$. As $\Tt$ is additive and  $\PW_n\not\sqsubseteq_\FO\Tt$ we deduce from \Cref{lem:plus_sl} that $\Tt_m+\PW_n\not\sqsubseteq_\FO\Tt$. Hence, $\Tt_m+\PW_n$ is incomparable with $\Tt$.
\end{proof}


%%%%%%%%%%%%%%%%%%


%\end{thm}
%\begin{proof}
%	We establish that $\PW_2\not\sqsubseteq_\FO\Tt$, from which $\TW_2\not\sqsubseteq_\FO \Tt$ immediately follows.
%	Assume for contradiction that $\PW_2\sqsubseteq_\FO\Tt$. 
%As $\PW_2$ is additive and \dnnc (\Cref{fact:non-copy-classes}), by \Cref{crl:slunion} there is an immersive transduction of $\PW_2$ in $\Tt$. In particular, there exists an integer $r$ such that the class $\{K_1\join P_n: n\in\mathbb N\}$ is the transduction of $\Tt_r$, which contradicts the property 
%		$\Pp\not\sqsubseteq_\FO\Tt_r$. Thus  $\PW_2\not\sqsubseteq_\FO\Tt$.
%
%
%
%We prove that the classes $\PW_n$ ($n\geq 2$) are incomparable with $\Tt$.
%The class $\Tt$ has unbounded linear cliquewidth, hence $\Tt\not\sqsubseteq_\FO\Hh$, and thus \mbox{$\Tt\not\sqsubseteq_\FO\PW_n$} for every integer $n$ (recall that a class $\Cc$ has bounded linear cliquewidth if and only if $\Cc\sqsubseteq_\FO \Hh$). As $\PW_2\not\sqsubseteq_\FO\Tt$ it follows that,  for $n\geq 2$,  $\PW_n\not\sqsubseteq_\FO\Tt$, thus $\PW_n$ and~$\Tt$ are incomparable. 
%	(This settles the case where $m=n+1$ as $\Tt_{n+1}+\PW_n=\PW_n$.)
%For $m>n+1$ the classes $\Tt_m$ and $\PW_n$ are additive and incomparable and $\Tt_m\sqsubset_\FO\Tt$. As 
%$\Tt$ is additive, essentially connected and incomparable with $\PW_n$ we deduce by \Cref{cor:incomp} that
%$\Tt_m+\PW_n$ is incomparable with $\Tt$.
%\end{proof}


%
%\BTT*
%
%\begin{proof}
%That $\Tt\not\sqsubseteq\BT$ directly follows from \Cref{lem:degree}.
%That the class of grids cannot be transduced in the class of cubic trees follows from the fact that cubic trees have bounded cliquewidth (i.e. $\BT\sqsubseteq_\FO\TP$) but grids do not. That the class of cubic trees cannot be transduced in the class of grids directly follows from \Cref{lem:growth}.
%\end{proof}


%\begin{lem}
%\label{lem:TnTnP}
%	$\Tt_n\cover_\FO\Tt_n\cup\Pp$.
%\end{lem}
%\begin{proof}
%	Let $\Cc$ be a class with 
%	$\Tt_n\sqsubset_\FO\Cc\sqsubseteq_\FO\Tt_n\cup\Pp$.
%	According to \Cref{fact:union} there exists a partition $\Cc_1\cup\Cc_2$ of $\Cc$ with $\Cc_1\sqsubseteq_\FO\Tt_n$ and $\Cc_2\sqsubseteq_\FO\Pp$. According to \Cref{thm:transpath}, $\Cc_2$ is a perturbation of a class $\Dd$ with bounded bandwidth. If $\Cc_2\not\equiv_\FO\Ee$ then $\Pp\sqsubseteq\Dd$ thus, as $\Dd\equiv_\FO\Cc$ and
%	 $\Tt_n\sqsubset_\FO\Cc$ by assumption we get $\Tt_n\cup\Pp\sqsubseteq\Cc$ thus $\Cc\equiv_\FO\Tt_n\cup\Pp$. It follows that $\Tt_n\cover_\FO\Tt_n\cup\Pp$.
%\end{proof}
%
%\begin{lem}
%\label{lem:PTnP}
%	If $n\geq 1$ then $\Tt_n\cup\Pp\cover_\FO\Tt_{n+1}\cup\Pp$.
%\end{lem}
%\begin{proof}
%	Let $\Cc$ be a class with 
%	$\Tt_n\cup\Pp\sqsubset_\FO\Cc\sqsubseteq_\FO\Tt_n\cup\Pp$.
%	According to \Cref{fact:union} there exists a partition $\Cc_1\cup\Cc_2$ of $\Cc$ with $\Cc_1\sqsubseteq_\FO\Tt_{n+1}$ and $\Cc_2\sqsubseteq_\FO\Pp$.
%	As $\Ee\cover_\FO\Tt_2\cover_\FO\dots\cover_\FO\Tt_{n+1}$ there exists an integer $m\leq n+1$ with $\Cc_1\equiv_\FO\Tt_m$.
%	If $m\leq n$ then $\Cc_1\cup\Cc_2\sqsubseteq \Tt_n\cup \Pp$, contradicting the assumption $\Tt_n\cup\Pp\sqsubset_\FO\Cc$.
%	Hence $m=n+1$ and we have $\Cc\equiv_\FO\Tt_{n+1}\cup\Pp$. 
%\end{proof}

%\begin{lem}
%\label{lem:Tn-T}
%	Assume $\Pp\not\sqsubseteq_\FO \Cc\sqsubset_\FO \Tt$. Then there exists some integer $n$ such that $\Cc\sqsubseteq_\FO \Tt_n$.
%\end{lem}
%\begin{proof}
%	We can assume that $\Cc$ is closed by disjoint unions and that the transduction from $\Tt$ is strongly local. Note that graphs in $\Cc$ have bounded diameter. It follows that we can assume that the pre-images in $\Tt$ also have bounded diameter hence belong to some $\Tt_n$.
%\end{proof}
%
%\begin{lem}
%\label{lem:T-PW2}
%	$\PW_2\not\sqsubseteq_\FO \Tt$.
%\end{lem}
%\begin{proof}
%	Assume for contradiction $\PW_2\sqsubseteq_\FO \Tt$. Let $\mathsf I(T_n^+)=nH_n$ where $H_n=K_1\join P_n$. We can assume that the interpretation is strongly local but then we deduce the interpretation of arbitrarily long paths in trees of height $r$, a contradiction.
%\end{proof}





%\begin{lem}
%\label{lem:GridBT}
%	The class of grids and the class of cubic trees are non comparable.
%\end{lem}
%\begin{proof}
%	As the hereditary closure of both classes are closed by disjoint unions, we can restrict ourselves to strongly local interpretations. Then cubic tree cannot be interpreted in grids as the number of vertices in a ball of radius $r$ grows exponentially fast in cubic trees and polynomially in grids.
%	Conversely, grids cannot be interpreted in cubic trees, as cubic trees have bounded rankwidth (i.e. can be interpreted in a tree order) and grids don't.
%\end{proof}



%\begin{conjecture}
%	There is no monadically stable class, in which every monadically stable class can be transduced.
%\end{conjecture}

%Figure~\ref{fig:Tsmall} displays a fragment of the transduction quasiorder. In this figure, $\mathcal E$ means edgeless, $\mathcal T_n$ stands for tree forest with height at most $n$, $\mathcal P$ for paths, $\mathcal{PW}_n$ for pathwidth at most $n$, $\mathcal{TW}_n$ for treewidth at most $n$, $\mathcal H$ for half-graphs, and $\mathcal{TP}$ for trivially perfect graphs.
%
%The transduction quasiorder of graph classes is intriguing, and some properties of this quasiorder have been studied in \cite{SODA_msrw,msrw}. 
%In particular, it is proved there that if a class $\Cc$ is a transduction of the class of half-graphs but has not transduction onto it (i.e. is monadically stable) then it is a transduction of a class with bounded pathwidth. In other words, just under $\mathcal H$ there is nothing else than the classes $\mathcal{PW}_n$.
%
%It is known that the quasiorder is strict on the chain
%$\mathcal E\sqsubset\mathcal T_2\sqsubset\dots\sqsubset\mathcal T_n\sqsubset\dots$ of classes of trees with bounded height. Note that the transductions of $\mathcal T_n$ are exactly the classes with shrubdepth at most $n$. In this section we prove that the chain 
%$\mathcal E\sqsubseteq\mathcal{P}\sqsubseteq\mathcal {PW}_2\sqsubseteq\dots\sqsubseteq\mathcal {PW}_n\sqsubset\dots$
%and $\mathcal E\sqsubseteq\mathcal{T}\sqsubseteq\mathcal{TW}_2\sqsubseteq\dots\sqsubseteq\mathcal {TW}_n\sqsubseteq\dots$
%is also strict.

%\subsection{The pathwidth hierarchy}
%\begin{figure}[ht]
%\begin{center}
%	\includegraphics[width=.3\textwidth]{hierarchy}
%\end{center}
%\caption{A fragment of the transduction quasiorder}
%\label{fig:hierarchy}
%\end{figure}

%\begin{lem}
%\label{lem:tnpw}
%	For every integer $n\geq 1$ we have 
%	$\Tt_{n+2}\not\sqsubseteq_\FO\PW_n$.
%%	For every non-negative integer $n$, there is no transduction from the class~$\PW_{n}$  onto the class $\Tt_{n+1}$.
%\end{lem}	
%%\begin{thm}
%%\label{thm:pw}
%%	For every non-negative integer $n$, there is no transduction from the class~$\mathcal{PW}_{n}$ of all graphs with pathwidth at most $n$ onto the class $\mathcal{PW}_{n+1}$ of all graphs with pathwidth at most $n+1$.
%%\end{thm}
%\begin{proof}
%	We prove this theorem by induction on $n$. The theorem is clear if $n=1$. Now assume that we have proved the statement for $n\geq 1$ and assume for contradiction that there is a transduction  from  $\PW_{n+1}$ onto $\Tt_{n+3}$.
%		The class $\PW_{n+1}$ is the monotone closure of the class $\mathcal{I}_{n+2}$ of interval graphs with clique number at most $n+2$. As the class  $\mathcal{I}_{n+2}$ has bounded star chromatic number, it follows from \Cref{lem:monotone} that there is a transduction from~$\mathcal{I}_{n+2}$ onto~$\PW_{n+1}$. Let $\mathsf T$ be the composition of these transductions, that is a transduction from $\mathcal{I}_{n+2}$ onto $\Tt_{n+3}$.
%	According to \Cref{thm:normal} the transduction~$\mathsf T$ is subsumed by the composition of a strongly local transduction $\mathsf T_0$ and a number of subset complementations. As $\Tt_{n+3}$ is closed by disjoint unions, we get that the subset complementations can be ignored and that $\mathsf T_0$ is a transduction from  $\mathcal{I}_{n+2}$ onto $\Tt_{n+3}$. 
%	 Now consider any graph $H\in \Tt_{n+1}$ and let $H'\in \Tt_{n+2}$ be the graph obtained from $2d$ copies of $H$ by adding a universal vertex $v$ and let $G$ be a graph in $\mathcal{I}_{n+2}$  such that $H'$ is a $\mathsf T$-transduction of $G$. As $\mathsf T_0$ is strongly local, we can assume that all the vertices of $G$ are at distance at most $d$ from $v$, where $d$ depends only on $\mathsf T_0$.  It is easily checked that there exists a path $P$ of length at most $2d$ of $G$ that dominates $G$, and such that $G-P\in\mathcal{I}_{n+1}$. By encoding the adjacencies in $G$ to the vertices of $P$ by a monadic expansion, we get that that there exists a transduction $\mathsf T_1$ (independent of our choice of $G$ and $H$) such that $H$ is a $\mathsf T_1$-transduction of $G-P$. In particular, $\mathsf T_1$ is a transduction from $\mathcal{PW}_{n}$ onto $\Tt_{n+2}$, what contradicts our induction hypothesis.
%\end{proof}
%
%So, in the transduction quasiorder $\sqsubset$, we have
%$$
%\mathcal E\sqsubset \mathcal P\sqsubset \mathcal{PW}_2\sqsubset\dots\sqsubset\mathcal{PW}_n\sqsubset\mathcal{PW}_{n+1}\sqsubset\dots\sqsubset\mathcal H.
%$$

%\subsection{The treewidth hierarchy (new stuff)}
%
%%We conjecture that the transduction quasiorder $\sqsubset$ is also strict on classes $\mathcal{TW}_n$.
%%
%%\begin{conjecture}
%%	For every non-negative integer $n$ there is no transduction from $\mathcal{TW}_n$ onto $\mathcal{TW}_{n+1}$.
%%\end{conjecture}
%
%Let $\mathsf T:\mathscr C\rightarrow\mathscr D$ be an existential transduction from a class $\mathscr C$ with bounded treewidth to a weakly sparse class $\mathscr D$.
%\begin{enumerate}
%	\item We can assume that there exists a finite set $\mathcal F$ of bi-rooted vertex-colored graphs $(F,u,v)$ such that the interpretation part of $\mathscr T$ connects vertices $x$ and $y$ if and only if there is some $A\subseteq G$ with $(G[A],x,y)$ isomorphic to some $(F,u,v)\in\mathcal F$. \textcolor{red}{Put to normal form for bounded expansion. In the source graph we have a closure of any set $A$ that is only linear in the size of $A$ and such that the transduction depends only on the closure.}
%	\item As $\mathcal D$ is weakly sparse we can assume $\mathcal F$ contains only connected graphs.
%	\item Let $\mathsf I$ be the corresponding interpretation. Assume $\mathsf I(G^+)=H$, where $G\in\mathscr C$, $H\in\mathscr D$, $G$ is connected, and $G^+$ is a monadic lift of $G$. Let $T$ be a tree-decomposition  of $G$ with width $k$. By changing the family $\mathcal F$ and the monadic lift if necessary, we can restrict to the minimal subtree of $T$ containing all the bags where a vertex in $V(H)$ appears first. 
%	\item If $H$ contains a long induced path $P$, then $V(P)$ has to include many vertices in some branch of $T$ (for otherwise we would bound the shrubdepth of $P$). In particular there is a part of $P$ that correspond to a sequence of vertices along a branch of $T$. \textcolor{red}{If we have a separator $S$ in the source, 
	%	and a long induced path in the target, then there is a connected component
	%	in the source that contains at least a $1/f(|S|)$ fraction of the path. The function $f$ is determined by the number of types over $S$, which can be reduced by 
	%	the existential normal form. In particular in bounded treewidth we get
	%	good bounds.}
%	\item If there is a long induced path $P_t$ in the target graph, then there is a long induced path $P_s$ in the source graph that contains many vertices of $P_t$ with bounded distance between two consecutive vertices of $P_t$ (on $P_s$). 
%	\item If $H$ is a universal graphs with pathwidth $k+1$ we can thus assume (by taking an induced subgraph) that each path in it 
%		goes along some branch of $T$.
%	\item From all the above, we deduce that we can restrict $T$ to a subtree with bounded pathwidth. It follows that we can take induced subgraphs of graphs in $\mathscr C$ with bounded pathwidth.
%	\item By the previous theorem the pathwidth has to be at least $k+1$, a contradiction.
%\end{enumerate}
%
%
%	Let $G$ be a graph with treewidth at most $k$, let $(X,T)$ be a tree decomposition of $G$ with width at most $k$, and let $X_0$ be a bag of the tree decomposition, which will serve as a root.
%
%	For every vertex $u\in V(G)$ we denote by $\Xi(u)$ the minimum bag in $T$ that contains $u$. Note $\Xi(u)$ can be alternatively defined as the infimum of all the bags that contain $u$.
%
%	Let $A$ be a subset of vertices of $G$. We denote by $T(A)$ 
%	the smallest connected subtree of $T$ that contains all the bags $\Xi(u)$ for $u\in A$. Alternative ly, 
%	$T(A)$ is the union of all the paths in $T$ linking two bags $\Xi(u)$ and $\Xi(v)$, for $u,v\in A$.
%	The {\em closure} $\overline{A}^T$ of $A$ is then defined as the union of the bags in $T(A)$.
%
%\begin{lem}
%	For every interpretation $\mathsf I:\mathscr C\rightarrow\mathscr D$, where $\mathscr C$ is a class of vertex-colored graphs with bounded treewidth, there exists a monadic lift operator $\Lambda$ and an interpretation $\mathsf I'$ such that for every graph $G\in\mathscr C$ with tree decomposition $(X,T)$ we have $\mathsf I(G)=\mathsf I'(\Lambda(G)[B])$, where $B=\overline{V(\mathsf I(G))}^T$.
%\end{lem}    
%
%\subsection{Conjectures}

%We conjecture that the classes $\mathcal{T}_n$ are the only class non-comparable with $\mathcal P$. These classes correspond to the classes with bounded shrub-depth. It follows that this conjecture can be stated as follows:
%
%
%\begin{conjecture}
%	A class has bounded shrub-depth if and only if it has no transduction onto the class of paths.
%\end{conjecture}
%Note that this conjecture is stronger than the conjecture stated in \cite{Ganian2017} where CMSO-transductions are considered instead of FO-transductions.
%
%
%The classes $\mathcal{PW}_n$ and $\mathcal{TW}_n$ are monadically stable classes. It is known that every class below $\mathcal H$ (that is: every monadically stable class with bounded linear cliquewidth) is a transduction of some $\mathcal{PW}_n$ \cite{SODA_msrw,msrw}.
%We conjecture that there is no monadically stable class between the classes with bounded treewidth and the class of trivially perfect graphs. This can be restated as follows:
%
%\begin{conjecture}[\cite{SODA_msrw,msrw}]
%	Every monadically stable class of graphs with a transduction onto trivially perfect graphs (that is: of bounded cliquewidth) is a transduction of a class with bounded treewidth.	
%\end{conjecture}




%Note that the classes of all graphs with cliquewidth at most $k$ for $k\geq 2$ collapse in the quasiorder with the class of trivially perfect graphs, as every class with bounded clique width is a transduction of the class of trivially perfect graphs and as the class of trivially perfect graphs is itself a transduction of the class of cographs, which has cliquewidth $2$. 


With the above results in hand, we obtain for $(\mathfrak C,\sqsubseteq_\FO)$ and $(\mathfrak A,\sqsubseteq_\FO)$ the structures sketched in \Cref{fig:TW2a,fig:TW2b}.

\begin{figure}[p]
	\begin{center}
		\includegraphics[height=.9\textheight]{narbo}	
		%\includegraphics[height=.44\textheight]{arbo2}
	\end{center}
	\caption{A fragment of $(\mathfrak C,\sqsubseteq_\FO)$. Thick edges are covers.}
	\label{fig:TW2a}
\end{figure}

\begin{figure}[p]
	\begin{center}
		\includegraphics[width=\textwidth]{arbo2}
	\end{center}
	\caption{A fragment of  $(\mathfrak A,\sqsubseteq_\FO)$. Thick edges are covers.}
	\label{fig:TW2b}
\end{figure}
\afterpage{\clearpage}


